CARMA: Fair and efficient bottleneck congestion management via non-tradable karma credits

This paper proposes a non-monetary traffic demand management scheme, named CARMA, as a fair solution to the morning commute congestion. We consider heterogeneous commuters traveling through a single bottleneck that differ in both the desired arrival time and Value of Time (VOT). We consider a generalized notion of VOT by allowing it to vary dynamically on each day (e.g., according to trip purpose and urgency), rather than being a static characteristic of each individual. In our CARMA scheme, the bottleneck is divided into a fast lane that is kept in free flow and a slow lane that is subject to congestion. We introduce a non-tradable mobility credit, named karma, that is used by commuters to bid for access to the fast lane. Commuters who get outbid or do not participate in the CARMA scheme instead use the slow lane. At the end of each day, karma collected from the bidders is redistributed, and the process repeats day by day. We model the collective commuter behaviors under CARMA as a Dynamic Population Game (DPG), in which a Stationary Nash Equilibrium (SNE) is guaranteed to exist. Unlike existing monetary schemes, CARMA is demonstrated, both analytically and numerically, to achieve a) an equitable traffic assignment with respect to heterogeneous income classes and b) a strong Pareto improvement in the long-term average travel disutility with respect to no policy intervention. With extensive numerical analysis, we show that CARMA is able to retain the same congestion reduction as an optimal monetary tolling scheme under uniform karma redistribution and even outperform tolling under a well-designed redistribution scheme. We also highlight the privacy-preserving feature of CARMA, i.e., its ability to tailor to the private preferences of commuters without centrally collecting the information.

==> figures-code/baseline-karma-redistribution-losers.tex <==
\hspace{-0.12\textwidth}
\begin{minipage}[t]{0.55\textwidth}
    \vspace{0pt}
    \raggedright
    \footnotesize
    
    % Traffic plot
    \def \tleft {33.42651pt}
    \def \tright {21.73213pt}
    \def \tleftt {15.36607pt}
    \def \trightt {5.64877pt}
    \includegraphics[trim={\tleft{} 0 \tright{} 0}]{tikz/baseline-karma-redistribution-losers-departures-fast}
    \hfill
    \includegraphics[trim={\tleftt{} 0 \trightt{} 0}]{tikz/baseline-karma-redistribution-losers-queue-time-fast}

    \def \tright {8.3707pt}
    \def \trightt {7.82932pt}
    \includegraphics[trim={\tleft{} 0 \tright{} 0}]{tikz/baseline-karma-redistribution-losers-departures-slow}
    \hfill
    \includegraphics[trim={\tleftt{} 0 \trightt{} 0}]{tikz/baseline-karma-redistribution-losers-queue-time-slow}
	
    \centering
    (a)
\end{minipage}
\hspace{1mm}
\vline
\hspace{1mm}
\begin{minipage}[t]{0.55\textwidth}
    \vspace{0pt}
    \raggedleft
    \footnotesize
    
    % Performance comparison plots
    \def \tleft {23.72046pt}
    \def \tright {23.72046pt}
    \def \tleftt {15.36607pt}
    \def \trightt {3.48428pt}
    \includegraphics[trim={\tleft{} 0 \tright{} 0}]{tikz/baseline-karma-redistribution-losers-t-q-bar}
    \hspace{7mm}
    \includegraphics[trim={\tleftt{} 0 \trightt{} 0}]{tikz/baseline-karma-redistribution-losers-c-q-bar}
	
    \centering
    (b)
    \captionof{figure}{Results for karma redistribution to slow lane commuters and zero bidders only.
    (a) Left: departure rate in $\karma$ versus $\toll$.
    Right: queuing delay over time.
    (b) Performance comparison of $\karma$ versus $\toll$ and $\nom$.}
    \label{fig:results-redistribution-losers}
\end{minipage}

==> figures-code/flow-chart.tex <==
\tikzstyle{startstop} = [rectangle, rounded corners, 
minimum width=1cm, 
minimum height=1cm,
text centered, 
inner sep = 0pt,
draw=black, 
fill=red!30]

\tikzstyle{io} = [trapezium, 
trapezium stretches=true, % A later addition
trapezium left angle=70, 
trapezium right angle=110, 
minimum width=3cm, 
minimum height=1cm, text centered, 
inner sep = 0pt,
draw=black, fill=blue!30]

\tikzstyle{process} = [rectangle, 
minimum size=1cm,  
text centered,
inner sep = 0pt,
inner ysep= 3pt,
draw=black, 
fill=orange!30]

\tikzstyle{decision} = [diamond,
aspect=1.25,
minimum width=1cm, 
minimum height=1cm, 
text centered, 
inner sep = 0pt,
draw=black, 
fill=green!30]

\tikzstyle{arrow} = [thick,->,>=stealth]

\makeatletter
\newcommand*{\centerfloat}{%
  \parindent \z@
  \leftskip \z@ \@plus 1fil \@minus \textwidth
  \rightskip\leftskip
  \parfillskip \z@skip}
\makeatother

\begin{figure}[htb]
    \centerfloat
    \begin{tikzpicture}[node distance=3.5cm]
        \scriptsize
        \node (curr-state) [startstop] {\begin{tabular}{c} \textbf{Commuter state} \\[1pt] $[u, k]$\end{tabular}};
        \node (action) [decision, right of=curr-state, xshift=0.3cm] {\begin{tabular}{c} \textbf{Commuter action} \\[1pt] $[t,b] \sim \pi_\tau[\cdot \mid u, k]$ \end{tabular}};
        \node (auction) [process, right of=action, xshift=0.3cm] {\begin{tabular}{c} \textbf{Auction outcome} \\[1pt] $o \in \{\fast, \slow\}$ \\[1pt] $o \sim \psi[\cdot \mid t, b]$\end{tabular}};
        \node (social-state) [startstop, above of=curr-state, yshift=-1cm] {\begin{tabular}{c} \textbf{Social state} \\[1pt] $(d,\pi)$ \end{tabular}};
        \node (action-dist) [process, above of=action, yshift=-1cm] {\begin{tabular}{c} \textbf{Distribution of actions} \\[1pt] $\nu$ \end{tabular}};
        \node (karma-transition) [io, right of=auction, xshift=0.3cm] {\begin{tabular}{c} \textbf{Karma transition} \\[1pt] $k^+ \sim \kappa[\cdot \mid k,t,b]$ \end{tabular}};
        \node (average-pay) [process, above of=karma-transition, yshift=-1cm] {\begin{tabular}{c} \textbf{Average payment} \\[1pt] $\pbar$ \end{tabular}};
        \node (reward) [io, below of=karma-transition, yshift=1.75cm] {\begin{tabular}{c} \textbf{Immediate reward} \\[1pt] $\zeta_\tau[u,t,b]$ \end{tabular}};
        \node (next-state) [startstop, right of=karma-transition] {\begin{tabular}{c} \textbf{Next state} \\[1pt] $[u^+, k^+]$ \end{tabular}};
        \node (VOT-transition) [process, above of=next-state, yshift=-1.75cm] {\begin{tabular}{c} \textbf{VOT transition} \\[1pt] $u^+ \sim \phi_\tau[\cdot \mid u]$ \end{tabular}};
        
        \coordinate[right = 0.5cm of next-state](empty1);
        \coordinate[below = 2.75cm of empty1](empty2);
        
        \draw [arrow] (curr-state) -- (action);
        \draw [arrow] (social-state) -- (action-dist);
        \draw [arrow] (action) -- (auction);
        \draw [arrow] (action-dist) -| (auction);
        \draw [arrow] (auction) |- (reward);
        \draw [arrow] (auction) -- (karma-transition);
        \draw [arrow] (action-dist) -- (average-pay);
        \draw [arrow] (average-pay) -- (karma-transition);
        \draw [arrow] (karma-transition) -- (next-state);
        \draw [arrow] (VOT-transition) -- (next-state);
        \draw [arrow] (next-state) -- (empty1) -- (empty2) -| (action);
        % node[below, pos=0.26] {Repeat}
        
        \end{tikzpicture}
    \caption{Flowchart of a commuter of type $\tau$.}
    \label{fig:flowchart}
\end{figure}

==> old_versions/introduction.tex <==
\section{Introduction}
% Start with a high level description of the traffic model and the relevance of policies. Then,  some studies on the fairness of the policies on heterogeneous populations. Discuss on high level different policies that have been implemented to decrease traffic congestion and then focus more on motivating why studying the single bottleneck model is important.
%  I would not mention karma here.
 
 
%  issue of congestion >> during commuting >> bottleneck
For decades, traffic congestion has been causing tremendous social cost to major cities around the world.
According to the INRIX $2019$ Global Traffic Scorecard report, drivers in the U.S. lost an average of 99 hours a year due to congestion, costing nearly $\$88$ billion in total. %\rev{TODO: it is a bit against the spirit of the paper to attach a monetary cost to congestion, I think reporting the loss of hours is enough}. 
The situation was even worse in the U.K., where drivers on average spent 115 hours in traffic~\cite{inrix2019global}. 
% existing policies: road pricing >> credit- and quantity-based schemes 
To manage rush hour traffic, a wide variety of tools have been proposed in the literature as well as implemented in practice. Among them, congestion pricing is the most widely known due to its theoretical efficiency. It suggests to internalize the cost of the negative externalities of individual travelers on the social cost~\cite{pigou1920economics,vickrey1969congestion,de2011traffic}. However, the classical congestion pricing is often arguably politically and socially unfair \cite{brands2020tradable} as it tends to favor wealthier travelers~\cite{arnott1994welfare,evans1992road,taylor2010addressing}.
Moreover, it is difficult to determine and implement the theoretically optimal tolls in real time~\cite{lindsey2006economists,yang2004trial,de2011traffic}.
As a result, most existing congestion pricing schemes are restricted to zone-, cordon- and facility-based schemes with flat rates during certain time windows~\cite{de2011traffic,cenedese:2022:EJC_bn_evs}.
% A particular facility-based scheme is HOT (high occupancy/toll) lane that can be used by carpoolers for free or by single drivers who pay the toll.  

Due to the limitations of congestion pricing, a growing attention has been drawn to alternative quantity- and credit-based approaches. The former directly limit the number of vehicles on the road, e.g., through license-plate rationing~\cite{wang2010traffic,han2010efficiency} or highway reservation~\cite{teodorovic2005highway,edara2008model}, while the latter assign a limited number of travel credits/permits to road users which can be traded in a monetary market~\cite{verhoef1997tradeable,teodorovic2008auction,yang2011managing,blum2022conceptualizing} \rev{(TODO: \cite{teodorovic2008auction} seems out of place)} or used as vouchers to pay for monetary tolls~\cite{kockelman2005credit}.
These approaches are preferable to classical congestion pricing as they avoid a net financial flow from road users to authorities, as well as mitigate some of the aforementioned practical difficulties~\cite{brands2020tradable,nie2013managing}.
% issue of unfairness
Nevertheless, these approaches fail to address the fairness issue. In fact, wealthy travelers can also take advantage of the credit-based schemes since they have a larger capacity to buy credits than others~\cite{xiao2013managing}. As a result, more transport capacities would be allocated to travelers with higher income levels. The license-plate rationing implemented in China is emblematic, indeed it has induced wealthy travelers to purchase additional vehicles worsening the problem rather than solving it~\cite{nie2017license}.
% , and indeed travelers with higher (monetary) \acrfull{VOT} benefit more in these schemes~\cite{xiao2013managing}.
 A fair and efficient mechanism should allocate these capacities based on the \emph{true urgency} of the travelers that could vary on a daily basis.
% In other words, the sought congestion management scheme should not discriminate against people with low-income but provide them with equal opportunities to reach their destinations in time when they are in urgent.
% \red{In this work, we attempt to clarify a misconception in the notion of \acrshort{VOT} classically measured in monetary units, and therefore inherently tied to the wealth of the travelers~\cite{borjesson2012income}.
Therefore, rather than quantifying \gls{VOT} as fixed and associated on a universal scale, viz. liked to a monetary value, we argue it should follow a dynamic process over days. 
% that it individually varies from one day to another according to a dynamic process.
% In our setting, a higher \gls{VOT} means that the individual has a more urgent need for congestion-free travel today in comparison to other days,
% % , and a more efficient allocation is one where those travelers who are more urgent today experience less delays.
% e.g., because it is late for an important appointment or must catch an important flight.
Despite of being intuitive, the daily variation in the \gls{VOT} has not been a focus of previous empirical studies~\cite{wardman1998value,zamparini2007meta,batley2010updating,borjesson2012income}.
While a clear correlation to trip distance and purpose (e.g., business, commuting, leisure) has been observed, few studies have investigated situational differences in the \gls{VOT} for the same distance and purpose (e.g., commuting from home to work).
A notable exception is~\cite{borjesson2012income} which reports a correlation to whether travelers must be exceptionally punctual.


In this study, we propose $\karma$, a novel congestion management scheme that uses non-monetary mobility credits called karma. Similar to other credit schemes, $\karma$ gives rise to a highly efficient traffic assignment without requiring any private information about the travelers. Differently, $\karma$ also manages to address the fairness issue discussed above because karma is not exchanged for and is completely decoupled from money. 
% We propose $\karma$: a novel congestion management scheme that is based on simple self-interested interactions facilitated through scarce road access tokens, called karma.
% These tokens are exchanged directly in the interactions and not in a monetary market.
% We demonstrate how $\karma$ gives rise to highly efficient and fair traffic assignments, without requiring access to the travelers' private preferences, and without resorting to any form of monetary pricing of the roads.

% \blue{At the same time, it should not require knowledge on the travelers preferences to be implemented. This work takes a disruptive approach by designing a novel congestion management scheme based on simple self-interested interactions among travelers that give rise to a desirable emerging behavior that created traffic decongestion.}




\subsection{Related work}
% Major literature that should be discussed:
% \begin{itemize}
%     \item  classical results on bottleneck model and tolling
%     \item difference between tolling and incentives 
%     \item line segmentation in order to decrease congestion. Use of a fast lane, e.g.,  only for AVs, or shared vehicles (increased occupancy). 
%     \item tradable  driving licences, performance compared to tolling advantages and disadvantages.  
% \end{itemize}
% For all the above it is good to stress the field studies or implementations already in place. Link in the US for priority lanes.

% bottleneck 
As a major contributor to urban traffic congestion, the morning commute problem has been studied extensively in the literature using the stylized bottleneck model~\cite{vickrey1969congestion,hendrickson1981schedule,daganzo1985uniqueness,arnott1990economics}, where commuters between a single origin-destination pair arrive at a bottleneck dynamically and form a queue due to its limited capacity. 
% bottleneck + tolling 
It is shown that, without intervention, the selfish choice of departure time by the commuters leads to costly traffic congestion. In contrast, a time-varying monetary toll, known as Vickrey's toll, is theoretically capable of achieving the socially optimal traffic assignment where the bottleneck congestion is completely eliminated. 
% is theoretically capable of eliminating any queuing at the bottleneck and achieving socially optimal traffic conditions. 
% A similar result holds regardless of the presence of user heterogeneity~\cite{arnott1988schedule}, route choice~\cite{arnott1990departure}, or the combination thereof~\cite{liu2011morning}.


% bottleneck + HOV/HOT/AV lane 
The original bottleneck model has been extended in various directions. One of them regards the design of a special lane that can only be used by a certain group of vehicles. The discussion started with the \gls{HOV} lanes that are exclusive for carpoolers~\cite{dahlgren1998high}, then extended to the \gls{HOT} lanes to increase the utilization rate of \gls{HOV} lanes meanwhile generating toll revenue~\cite{dahlgren2002high}. It is found that both \gls{HOV} and \gls{HOT} promote carpooling and reduce social cost, and converting an \gls{HOV} lane into an \gls{HOT} lane may further increase the carpool ratio~\cite{zhong2020dynamic}. Recent studies also discuss the capacity allocation between regular and \gls{HOV} lanes~\cite{wang2019optimal}. 
Moreover, it has been recently proposed to dedicate lanes for connected and autonomous vehicles, driven by their potential in increasing road capacity~\cite{lamotte:2016:bottleneck_w_AVs}.   

% bottleneck + tradable credit 
% add Daganzo (2000)
Another line of research examines the performance of tradable credits in managing traffic during the rush hours. 
In \cite{xiao2013managing}, Vickrey's toll is substituted by a time-varying credit charging scheme coupled with a daily initial allocation of credits. When late arrival is not allowed, the authors have shown that  an optimal scheme could achieve the system optimum and eliminate congestion. 
Yet, similar to Vickrey's toll, a time-varying charging scheme could be challenging to compute in practice. Hence, a step-wise charging scheme is proposed in \cite{nie2015new}. 
Specifically, travelers who pass the bottleneck during the peak time either pay a fixed amount of credits or a higher toll, while those traveling during the off-peak are rewarded with credits.
% The optimal ratio between credits charged and rewarded, which is equal (or close) to $1$ in various model configurations, can obtain a $50\%$ reduction in the  total travel delay.
The analysis is extended in~\cite{nie2013managing} to consider elastic demand with alternative mode choice.
Although the tradable credit scheme solves several shortcomings of congestion pricing, the authority still needs to design the credit charging scheme. The design is hardly optimal since the private information of travelers, e.g., their \acrshort{VOT}, is often not available.
Moreover, the monetary trading of credits leads to favoring high income travelers, as discussed above.


% auction-based congestion pricing
In essence, traffic demand management regards the efficient allocation of the scarce transport resources to the transport users. Accordingly, a few studies introduced auctions as a mechanism design approach to perform this resource allocation under private user information.
In~\cite{teodorovic2008auction}, a one-shot auction is designed  to determine the times and duration each traveler may visit the downtown area. The optimal allocation is solved via a combinatorial optimization problem, albeit the bidding strategy of each traveler is not explicitly modeled (the bids are considered exogenous).  
A similar combinatorial auction is proposed in~\cite{zhou2014combinatorial} to allocate traffic in a more general network. To induce truthful reporting of private values, the Vickrey-Clarke-Groves (VCG) mechanism is used to compute the payment of each traveler for its assigned path. 
The same mechanism has been introduced to the optimal pricing and matching in ride-sharing~\cite{kleiner2011mechanism,zhang2015discounted,li2020pricing} and car-sharing~\cite{hara2018car,lam2015combinatorial}. 
A few auction-based mechanisms are also proposed to manage the bottleneck traffic. In~\cite{wang2018trading}, the peak period is divided into small intervals and travelers may bid for each interval over multiple days. 
% Accordingly, a multi-periods bottleneck permit trading mechanism is developed that combines a dynamic auction and a capacity control. 
To promote ride-sharing, \cite{li2022auction} designs a mechanism that jointly determines the permit allocation and the shared trip assignment.
% , which are solved from a trilateral matching problem. 
Since the auctions in all of these approaches are monetary, they are also subject to the fairness issue discussed above.

The sensitivity towards the use of money is not exclusive to traffic demand management.
In the economics literature, a significant body of works has regarded the design of mechanisms without money~\cite{schummer2007mechanism}, 
such as organ donations~\cite{roth2004kidney,sonmez2020incentivized,kim2021organ} and college admissions~\cite{gale1962college,hylland1979efficient}.
% This includes mechanisms for organ donations~\cite{roth2004kidney,sonmez2020incentivized,kim2021organ},
% college admissions~\cite{gale1962college,hylland1979efficient}, and the allocation of oversubscribed course seats~\cite{sonmez2010course,budish2012multi}.
Despite of some successes, non-monetary mechanisms are in general difficult to design in a truth-revealing manner since they cannot rely on a general incentive instrument like money~\cite{gibbard1973manipulation,satterthwaite1975strategy}.
However, when the resource is repeatedly contested, a few studies have shown that this can be leveraged to incentivize truthfulness~\cite{balseiro2019multiagent,guo2020dynamic}.
% The core enabling 
The core principle is to let the resource users trade-off between immediate and future access to the resource.
In recent work, this principle is formalized in a practical mechanism, called karma mechanism,
% based on biding for the resource~\cite{elokda2022self}.
in which users are allocated karma points to bid for the resource, and karma is transferred directly from those who manage to acquire the resource to those who yield it~\cite{elokda2022self}.
This provides the departure point for the present study, which applies karma mechanisms to bottleneck congestion management.
% A rigorous game-theoretical model is developed to study these mechanisms, and provides the theoretical foundation of the present study.

\subsection{Paper contribution}
% Discuss the limitations of the proposed approaches:
% \begin{itemize}
%     \item they rely on money that is intrinsically unfair. 
%     \item optimal tolling policies usually require the knowledge of the parameters in the users' cost. May be difficult to estimate.
%     \item tolling requires that the users pays for the negative externalities it produces. There is no redistribution to the community, that happens instead for karma. \item trading is similar to karma, but having to pay for the permit via money means that there is still unfairness to low-income people. Some authors try to counterbalance the problem via heuristic. In our case fairness is intrinsic. 
% \end{itemize}



% brief summary
In this study, a bottleneck model is constructed to represent the dynamic traffic during rush hour. The model consists of a fast lane operated at or below capacity and a slow lane subject to congestion.
Our proposed scheme, called $\karma$, regulates access to the fast lane as follows.
All commuters are given an equal initial endowment of karma points which they use to bid on accessing the fast lane on a daily basis, based on their current \acrshort{VOT}.
% On each day, travelers bid, based on their current karma balance and \acrshort{VOT}, to gain access to the fast lane.
At the end of each day, karma is transferred directly from commuters who entered the fast lane to those who entered the slow lane.
In sharp contrast to existing credit and monetary auction schemes, access to the fast lane is solely enabled by karma and not money and there exists no monetary market to trade karma.
% In contrast to previous work on lane segmentation, access to the fast lane is not restricted to any kind of commuters (e.g., carpoolers or CAVs).
% , while demonstrably maintaining the fairness of this access.
We demonstrate that this non-monetary instrument fosters a fair and efficient use of the fast lane capacity.
This could encourage dedicating more capacity to the fast lane and assist in further decongestion.
\rev{Moreover, we demonstrate that through a well-designed, time-varying karma redistribution scheme, $\karma$ could further reduce the congestion in the slow lane, thereby outperforming the optimal decongestion in a monetary tolling of the fast lane.}
% Instead, all travelers have the opportunity to enter the fast lane and their preference is reflect on the karma bids. This idea is similar to tradable credit and other auction-based mechanisms, though karma is not associated with money, i.e., no one can purchase additional karmas. 
% % Different from existing work, this study proposes a non-monetary mechanism based on Karma games, firstly introduced in~\cite{elokda2022self}, to manage the traffic congestion during morning commute. Travelers participating in the mechanism initially receive a certain amount of credits, named karmas, and use them for daily commute. It is important to stress that karma is not associated with money since no user can purchase additional karma. 
% Therefore, karma is a scarce resource and we will show this feature fosters fairness in terms of the use of transport capacity.
% % exploitation of the transportation infrastructure.


% A bottleneck model is constructed to represent the dynamic traffic during rush hour. The model consists of a fast lane operated equal or below capacity and a slow lane subject to congestion. On each day, Karma users  bid, based on their current Karma balance and urgency level, to gain  access to the fast lane. Hence, a jointly decision on departure time and bid is made by each traveler in anticipation of other travelers' actions as well as the future travel. During a time interval the Karma payed by those entering the fast lane is automatically redistributed to those that had to use the slow lane, and thus experienced congestion. 

The main contributions of the paper can be summarized as follows:
\begin{itemize}
    \item  we formalize $\karma$ as a dynamic population game~\cite{elokda2021dynamic} which rigorously incorporates the commuters' strategic behavior.
    We prove that a \acrfull{SNE} exists in this game (Section~\ref{sec:karma-bottleneck});
    % Moreover, we show the outcome of such a game is a stationary Nash equilibrium and prove its existence.
    % Moreover, we prove the existence  of the equilibrium of such a game and show that is is a stationary Nash equilibrium;
    \item through numerical analysis, we demonstrate the efficiency of $\karma$ in reducing the bottleneck congestion, which is close to the theoretical efficiency of an optimal monetary tolling scheme \rev{of the fast lane} (Section~\ref{sec:numerical-analysis});
    % traffic decongestion of the Karma mechanism is comparable to the one obtained via monetary tolling;
    \item we further analyze the fairness of $\karma$ from the perspective of individual commuters with heterogeneous \rev{desired arrival times} and \acrshort{VOT} processes and show that it \rev{successfully addresses the fairness issue of existing monetary and credit-based policies. In particular, $\karma$ leads to a perfectly equitable allocation of the fast lane when commuters are heterogeneous with respect to monetary income (Section~\ref{subsec:heterogeneous-income}). For more general heterogeneity, we show that all commuter types experience a strict Pareto improvement under $\karma$ with respect to no policy intervention (Sections~\ref{subsubsec:pareto-improvement}, \ref{subsec:heterogeneous-income}--\ref{subsec:heterogeneous-tstar});}
    % outperforms the classical monetary policy.
    % the proposed approach from the point of view of the single individual and show that the Karma mechanism trumps classical monetary policies.
    \item \rev{we test the robustness of $\karma$ to heterogeneous desired arrival times, demonstrating its ability to adapt to heterogeneous demands in a decentralized manner (Section~\ref{subsec:heterogeneous-tstar}).
    To be robust against small subpopulations that desire to arrive outside the congested period and therefore should not take part in the system, we propose the simple intervention of a karma cap beyond which commuters do not get redistributed more karma.
    We demonstrate that this successfully eliminates irrelevant users in a decentralized manner and without affecting the efficiency of the scheme;}

    \item \rev{lastly, we showcase how the design degree of freedom of the karma redistribution can be utilized to cause further decongestion in the slow lane, by considering a time-varying karma redistribution scheme (Section~\ref{sec:non-uniform-redistribution}).
    With this scheme, $\karma$ outperforms the efficiency of an optimal monetary tolling scheme of the fast lane.}
\end{itemize}

\rev{The main benefits of $\karma$ with respect to existing schemes is further summarized in Figure~XXX. TODO: the spider web figure}



\subsection{Notation}
Let $a,d \in D\subseteq \Nat$  and let $c \in C\subseteq \Real^n$, then
for a function $f : D \times C \rightarrow \Real$, we distinguish discrete and continuous arguments through the notation $f[d](c)$.
Alternatively, we write $f : C \rightarrow \Real^{|D|}$ as the vector-valued function $f(c)$, with $f[d](c)$ denoting its $d^\textup{th}$ element.
Similarly, $g[a \mid d](c)$ denotes the conditional probability of $a$ given $d$ and $c$. 
Specifically, $g[d^+ \mid d](c)$ denotes one-step transition probabilities for $d$.
We denote by $p \in \Delta(D):=\left\{\left. \sigma \in \Real_+^{|D|} \right\rvert \sum_{d \in D} \sigma[d] = 1 \right\}$ a probability distribution over the elements of $D$, with $p[d]$ denoting the probability of element $d$.
Finally, when considering heterogeneous commuter types, we denote by $x_\tau$ a quantity associated to type $\tau$.

==> old_versions/introduction_v2.tex <==
\section{Introduction}
\label{sec:intro}
% Start with a high level description of the traffic model and the relevance of policies. Then,  some studies on the fairness of the policies on heterogeneous populations. Discuss on high level different policies that have been implemented to decrease traffic congestion and then focus more on motivating why studying the single bottleneck model is important.
%  I would not mention karma here.
 
 
%  issue of congestion >> during commuting >> bottleneck
For decades, traffic congestion has been causing tremendous social cost to major cities around the world.
According to the INRIX $2019$ Global Traffic Scorecard report, drivers in the U.S. lost an average of 99 hours a year due to congestion, costing nearly $\$88$ billion in total. %\rev{TODO: it is a bit against the spirit of the paper to attach a monetary cost to congestion, I think reporting the loss of hours is enough}. 
The situation was even worse in the U.K., where drivers on average spent 115 hours in traffic~\cite{inrix2019global}. 
% existing policies: road pricing >> credit- and quantity-based schemes 
To manage rush hour traffic, a wide variety of tools have been proposed in the literature as well as implemented in practice. Among them, congestion pricing is the most widely known due to its theoretical efficiency. It suggests internalizing the cost of the negative externalities of individual travelers on the social cost~\cite{pigou1920economics,vickrey1969congestion,de2011traffic}. However, the classical congestion pricing is often arguably politically and socially unfair \cite{brands2020tradable} as it tends to favor wealthier travelers~\cite{arnott1994welfare,evans1992road,taylor2010addressing}.
Moreover, it is difficult to determine and implement the theoretically optimal tolls in real time~\cite{lindsey2006economists,yang2004trial,de2011traffic}.
As a result, most existing congestion pricing schemes are restricted to zone-, cordon- and facility-based schemes with flat rates during certain time windows~\cite{de2011traffic,cenedese:2022:EJC_bn_evs}.
% A particular facility-based scheme is HOT (high occupancy/toll) lane that can be used by carpoolers for free or by single drivers who pay the toll.  

Due to the limitations of congestion pricing, growing attention has been drawn to alternative quantity- and credit-based approaches. The former directly limit the number of vehicles on the road, e.g., through license-plate rationing~\cite{wang2010traffic,han2010efficiency} or highway reservation~\cite{teodorovic2005highway,edara2008model}, while the latter assign a limited number of travel credits/permits to road users which can be traded in a monetary market~\cite{verhoef1997tradeable,yang2011managing,blum2022conceptualizing} or used as vouchers to pay for monetary tolls~\cite{decorla1994applying,daganzo1995pareto,decorla2000fair,kockelman2005credit}.
These approaches are preferable to classical congestion pricing as they avoid a net financial flow from road users to authorities, as well as mitigate some of the aforementioned practical difficulties~\cite{brands2020tradable,nie2013managing}.
% issue of unfairness
Nevertheless, they fail to fundamentally address the fairness issue. In fact, wealthy travelers persist in being favored by credit-based schemes since they have a larger capacity to buy or bypass credits than others~\cite{xiao2013managing}. As a result, more transport capacities would be allocated to travelers with higher income levels. The license-plate rationing implemented in China is emblematic, indeed it has induced wealthy travelers to purchase additional vehicles worsening the problem rather than solving it~\cite{nie2017license}.
% , and indeed travelers with higher (monetary) \acrfull{VOT} benefit more in these schemes~\cite{xiao2013managing}.

A fair and efficient mechanism should allocate transport capacities based on the \emph{true urgency} of the travelers that could vary on a daily basis.
% In other words, the sought congestion management scheme should not discriminate against people with low-income but provide them with equal opportunities to reach their destinations in time when they are in urgent.
% \red{In this work, we attempt to clarify a misconception in the notion of \acrshort{VOT} classically measured in monetary units, and therefore inherently tied to the wealth of the travelers~\cite{borjesson2012income}.
Therefore, rather than quantifying \gls{VOT} as \tbc{static}, and associated to a universal scale, viz. linked to a monetary value, we \tbc{model it as a} dynamical process over days. 
% that it individually varies from one day to another according to a dynamic process.
% In our setting, a higher \gls{VOT} means that the individual has a more urgent need for congestion-free travel today in comparison to other days,
% % , and a more efficient allocation is one where those travelers who are more urgent today experience less delays.
% e.g., because it is late for an important appointment or must catch an important flight.
Despite of being intuitive, the daily variation in the \gls{VOT} has not been a focus of previous empirical studies~\cite{wardman1998value,zamparini2007meta,batley2010updating,borjesson2012income}.
While a clear correlation to trip distance and purpose (e.g., business, commuting, leisure) has been observed, few studies have investigated situational differences in the \gls{VOT} for the same distance and purpose (e.g., commuting from home to work).
A notable exception is~\cite{borjesson2012income} which reports a correlation to whether travelers must be exceptionally punctual.


In this study, we propose $\karma$, a novel congestion management scheme that uses non-monetary mobility credits called karma to bridge the shortcomings of previously proposed schemes. 
% Similar to other credit schemes, $\karma$ gives rise to a highly efficient traffic assignment without requiring any private information about the travelers. Differently, and more importantly, $\karma$ manages to address the fairness issue discussed. 
Under $\karma$, the bottleneck is divided into two lanes: a fast lane that is kept in free flow and a slow lane that is subject to congestion. $\karma$ regulates access to the fast lane as follows. All commuters are initially endowed with an equal number of non-tradable credits called karma which they use to bid for the fast lane on a daily basis. At the end of each day, karma collected from the bidding is redistributed to the commuters. 
\kz{Similar to other credit schemes, $\karma$ gives rise to a highly efficient traffic assignment meanwhile being revenue neutral. Differently, $\karma$ manages to address the fairness issues discussed above.
Namely, since karma is completely decoupled from money, commuters of heterogeneous income classes (i.e., heterogeneous average \gls{VOT}) experience the same average travel time and cost reduction under $\karma$, a property we hereafter refer to as \emph{equity with respect to heterogeneous income}.
Moreover, under more general heterogeneity in the \gls{VOT} processes of the commuters, $\karma$ guarantees a \emph{strong Pareto improvement} in the average travel costs with respect to no policy intervention.
Finally, since the number of credits required to enter the fast lane is determined by the bidding process rather than a central planner, $\karma$ effectively tailors to the private preferences of the commuters without requiring centralized information.

This Pareto-improving strategy has been discussed in \cite{daganzo2000pareto}, though $\karma$ provides a more practical scheme with minimum intervention of the authority.
}


The key properties of $\karma$ and the main contributions of this paper are summarized as follows.

\begin{itemize}
    \item We conceptualize $\karma$ and formulate it as a dynamic population game~\cite{elokda2021dynamic} that describes the commuters' strategic behaviors. The existence of a \acrfull{SNE} is also guaranteed under mild conditions (Proposition~\ref{prop:sne-existence}).

    \item We prove that $\karma$ ensures a strict Pareto improvement with respect to no policy intervention in terms of fairness in allocating the fast lane among heterogeneous commuters and efficiency in reducing system cost (Proposition~\ref{prop:strict-pareto}). 
    
    \item Through numerical analysis, we demonstrate that $\karma$ achieves the same performance in congestion mitigation compared to the optimal monetary tolling scheme and it can even outperform the optimal tolling with a well-designed karma redistribution scheme. On the other hand, $\karma$ performs a more equitable allocation of fast lane capacity compared to the optimal tolling scheme or tradable credit.    

    \item We also showcase the robustness of $\karma$ towards different user heterogeneity (e.g., VOT and desired arrival time). This further emphasizes the privacy-preserving feature of $\karma$, i.e., no coordination or exchange of information is needed to obtain the equilibrium. 

\end{itemize}

Figure~\ref{fig:spdergraph} provides a qualitative comparison between the monetary tolling, tradable credit, and $\karma$. \kz{(short description to be added here. though it is not clear to me why tolling has half privacy (should be no privacy), tradable credit is half in all metrics (should be full effect, no fairness and full privacy). also, it is better to say efficiency instead of effect?)}
% We propose in Figure~\ref{fig:spdergraph} a qualitative representation of the different benefits and drawbacks of adopting different policies based on monetary tolling, tradable credits, or \karma. 
\begin{figure}[htb]
\centering
\includegraphics[clip,trim=0 0 0 10, width=\textwidth]{figures/SpiderGraph.pdf}
\caption{A qualitative depiction of the performances of  existing congestion management schemes (on the left) and \karma  (on the right).}
\label{fig:spdergraph}
\end{figure}



% above because karma is not exchanged for and is completely decoupled from money. 
% We propose $\karma$: a novel congestion management scheme that is based on simple self-interested interactions facilitated through scarce road access tokens, called karma.
% These tokens are exchanged directly in the interactions and not in a monetary market.
% We demonstrate how $\karma$ gives rise to highly efficient and fair traffic assignments, without requiring access to the travelers' private preferences, and without resorting to any form of monetary pricing of the roads.

% \blue{At the same time, it should not require knowledge on the travelers preferences to be implemented. This work takes a disruptive approach by designing a novel congestion management scheme based on simple self-interested interactions among travelers that give rise to a desirable emerging behavior that created traffic decongestion.}

The remaining of this paper is organized as follows. We first review the related work on bottleneck congestion management in Section~\ref{sec:review}. In Section~\ref{sec:karma-bottleneck}, we detail the implementation of $\karma$, present the game-theoretic formulation and discuss its key analytical properties. The results of the numerical experiments are summarized in Section~\ref{sec:numerical-analysis}. Finally, we conclude this paper in Section~\ref{sec:conclusion}. 


\section{Related work}
\label{sec:review}
% Major literature that should be discussed:
% \begin{itemize}
%     \item  classical results on bottleneck model and tolling
%     \item difference between tolling and incentives 
%     \item line segmentation in order to decrease congestion. Use of a fast lane, e.g.,  only for AVs, or shared vehicles (increased occupancy). 
%     \item tradable  driving licences, performance compared to tolling advantages and disadvantages.  
% \end{itemize}
% For all the above it is good to stress the field studies or implementations already in place. Link in the US for priority lanes.

% bottleneck 
As a major contributor to urban traffic congestion, the morning commute problem has been studied extensively in the literature using the stylized bottleneck model~\cite{vickrey1969congestion,hendrickson1981schedule,daganzo1985uniqueness,arnott1990economics}, where commuters between a single origin-destination pair arrive at a bottleneck dynamically and form a queue due to its limited capacity. 
% bottleneck + tolling 
It is shown that, without intervention, the selfish choice of departure time by the commuters leads to costly traffic congestion. In contrast, a time-varying monetary toll, known as Vickrey's toll, is theoretically capable of achieving the socially optimal traffic assignment where the bottleneck congestion is completely eliminated. 
% is theoretically capable of eliminating any queuing at the bottleneck and achieving socially optimal traffic conditions. 
% A similar result holds regardless of the presence of user heterogeneity~\cite{arnott1988schedule}, route choice~\cite{arnott1990departure}, or the combination thereof~\cite{liu2011morning}.


% bottleneck + HOV/HOT/AV/FAIR lane 
The original bottleneck model has been extended in various directions. One of them regards the design of a special lane that can only be used by a certain group of vehicles. The discussion started with the \gls{HOV} lanes that are exclusive for carpoolers~\cite{dahlgren1998high}, then extended to the \gls{HOT} lanes to increase the utilization rate of \gls{HOV} lanes meanwhile generating toll revenue~\cite{dahlgren2002high}. It is found that both \gls{HOV} and \gls{HOT} promote carpooling and reduce social cost, and converting an \gls{HOV} lane into an \gls{HOT} lane may further increase the carpool ratio~\cite{zhong2020dynamic}. Recent studies also discuss the capacity allocation between regular and \gls{HOV} lanes~\cite{wang2019optimal}. 
% \kz{Another lane separation scheme is proposed in \cite{decorla2000fair}, where users of the fast lane are tolled and those using the regular lane are compensated with credits that can be used to pay for the fast-lane toll in future trips.}
Moreover, it has been recently proposed to dedicate lanes for connected and autonomous vehicles, driven by their potential in increasing road capacity~\cite{lamotte:2016:bottleneck_w_AVs}.   

% bottleneck + rationing/tradable credit 

Another line of research examines the performance of tradable credits in managing traffic during rush hours. 
In \cite{xiao2013managing}, Vickrey's toll is substituted by a time-varying credit charging scheme coupled with a daily initial allocation of credits. When late arrival is not allowed, the authors have shown that  an optimal scheme could achieve the system optimum and eliminate congestion. 
Yet, similar to Vickrey's toll, a time-varying charging scheme could be challenging to compute in practice. Hence, a step-wise charging scheme is proposed in \cite{nie2015new}. 
Specifically, travelers who pass the bottleneck during the peak time either pay a fixed amount of credits or a higher toll, while those traveling during the off-peak are rewarded with credits.
% The optimal ratio between credits charged and rewarded, which is equal (or close) to $1$ in various model configurations, can obtain a $50\%$ reduction in the  total travel delay.
The analysis is extended in~\cite{nie2013managing} to consider elastic demand with alternative mode choice.
Although the tradable credit scheme solves several shortcomings of congestion pricing \kz{and partially addresses the equity issue~\cite{seshadri2022congestion}}, the authority still needs to design the credit charging scheme. The design is hardly optimal since the private information of travelers, e.g., their \acrshort{VOT}, is often not available.
Moreover, the monetary trading of credits still leads to favoring high-income travelers, as discussed above.
\rev{Other credit-based schemes do not allow the monetary trading of credits, which are instead used as vouchers to pay for monetary tolls~\cite{decorla1994applying,daganzo1995pareto,decorla2000fair,kockelman2005credit}.
In~\cite{decorla2000fair}, a lane separation scheme is proposed where travelers of the fast lane are tolled, and travelers of the regular lane are compensated with credits that can be used to pay for future fast lane tolls.
A systemic advantage to high-income travelers persists, who have a larger capacity to pay for tolls without the need for credits.
}

% auction-based congestion pricing
In essence, traffic demand management regards the efficient allocation of scarce transport resources to transport users. Accordingly, a few studies introduced auctions as a mechanism design approach to perform this resource allocation under private user information.
In~\cite{teodorovic2008auction}, a one-shot auction is designed  to determine the times and duration each traveler may visit the downtown area. The optimal allocation is solved via a combinatorial optimization problem, albeit the bidding strategy of each traveler is not explicitly modeled (the bids are considered exogenous).  
A similar combinatorial auction is proposed in~\cite{zhou2014combinatorial} to allocate traffic in a more general network. To induce truthful reporting of private values, the Vickrey-Clarke-Groves (VCG) mechanism is used to compute the payment of each traveler for its assigned path. 
The same mechanism has been introduced to the optimal pricing and matching in ride-sharing~\cite{kleiner2011mechanism,zhang2015discounted,li2020pricing} and car-sharing~\cite{hara2018car,lam2015combinatorial}. 
A few auction-based mechanisms are also proposed to manage the bottleneck traffic. In~\cite{wang2018trading}, the peak period is divided into small intervals and travelers may bid for each interval over multiple days. 
% Accordingly, a multi-periods bottleneck permit trading mechanism is developed that combines a dynamic auction and a capacity control. 
To promote ride-sharing, \cite{li2022auction} designs a mechanism that jointly determines the permit allocation and the shared trip assignment.
% , which are solved from a trilateral matching problem. 
Since the auctions in all of these approaches are monetary, they are also subject to the fairness issue discussed above.

The sensitivity towards the use of money is not exclusive to traffic demand management.
In the economics literature, a significant body of works has regarded the design of mechanisms without money~\cite{schummer2007mechanism}, 
such as organ donations~\cite{roth2004kidney,sonmez2020incentivized,kim2021organ} and college admissions~\cite{gale1962college,hylland1979efficient}.
% This includes mechanisms for organ donations~\cite{roth2004kidney,sonmez2020incentivized,kim2021organ},
% college admissions~\cite{gale1962college,hylland1979efficient}, and the allocation of oversubscribed course seats~\cite{sonmez2010course,budish2012multi}.
Despite of some successes, non-monetary mechanisms are in general difficult to design in a truth-revealing manner since they cannot rely on a general incentive instrument like money~\cite{gibbard1973manipulation,satterthwaite1975strategy}.
However, when the resource is repeatedly contested, a few studies have shown that this can be leveraged to incentivize truthfulness~\cite{balseiro2019multiagent,guo2020dynamic}.
% The core enabling 
The core principle is to let the resource users trade-off between immediate and future access to the resource.
In recent work, this principle is formalized in a practical mechanism, called karma mechanism,
% based on biding for the resource~\cite{elokda2022self}.
in which users are allocated karma points to bid for the resource, and karma is transferred directly from those who manage to acquire the resource to those who yield it~\cite{elokda2022self}.
\kz{A similar mechanism has been recently explored in the context of static traffic routing using a centrally controlled pricing scheme \cite{salazar2021urgency}, while in the present study, we consider the dynamic bottleneck congestion with no centralized control.}
% This provides the departure point for the present study, which applies karma mechanisms to bottleneck congestion management.
% A rigorous game-theoretical model is developed to study these mechanisms, and provides the theoretical foundation of the present study.


% \subsection{Paper contribution}
% % Discuss the limitations of the proposed approaches:
% % \begin{itemize}
% %     \item they rely on money that is intrinsically unfair. 
% %     \item optimal tolling policies usually require the knowledge of the parameters in the users' cost. May be difficult to estimate.
% %     \item tolling requires that the users pays for the negative externalities it produces. There is no redistribution to the community, that happens instead for karma. \item trading is similar to karma, but having to pay for the permit via money means that there is still unfairness to low-income people. Some authors try to counterbalance the problem via heuristic. In our case fairness is intrinsic. 
% % \end{itemize}
% % brief summary
% In this study, a bottleneck model is constructed to represent the dynamic traffic during rush hour. We propose to split the road in a fast lane operated at, or below, capacity and a slow lane that might be subject to congestion.
% Our proposed scheme, called $\karma$, regulates access to the fast lane as follows.
% All commuters are given an equal initial endowment of non-tradable karma points which they use to bid on accessing the fast lane on a daily basis, based on their current \acrshort{VOT}.
% % On each day, travelers bid, based on their current karma balance and \acrshort{VOT}, to gain access to the fast lane.
% At the end of each day, karma is transferred directly from commuters who entered the fast lane to those who entered the slow lane.
% In sharp contrast to existing credit and monetary auction schemes, access to the fast lane is solely enabled by karma and not money and there exists no monetary market to trade karma.
% % We demonstrate that this non-monetary instrument fosters a fair and efficient use of the fast lane capacity.
% % This could encourage dedicating more capacity to the fast lane and assist in further decongestion.
% % \rev{Moreover, we demonstrate that through a well-designed, time-varying karma redistribution scheme, $\karma$ could further reduce the congestion in the slow lane, thereby outperforming the optimal decongestion in a monetary tolling of the fast lane.}
% In the following, we summarize the main contributions of the paper and interesting features of \karma.
% \begin{itemize}
%     \item  We formalize $\karma$ as a dynamic population game~\cite{elokda2021dynamic}  rigorously incorporating the commuters' strategic behavior, and prove the existence of a \acrfull{SNE}(Section~\ref{sec:karma-bottleneck}).
%     \item For general heterogeneity in the commuters preferences, we prove that all commuters experience a strict Pareto improvement under $\karma$ with respect to no policy intervention (Sections~\ref{subsubsec:pareto-improvement}, \ref{subsec:heterogeneous-income}--\ref{subsec:heterogeneous-tstar}).
%     \item We analyze the fairness of $\karma$ from the perspective of individual commuters with heterogeneous desired arrival times and \acrshort{VOT} processes and show that it successfully addresses the fairness issue of existing monetary and credit-based policies. In particular, $\karma$ leads to a perfectly equitable allocation of the fast lane when commuters are heterogeneous with respect to monetary income (Section~\ref{subsec:heterogeneous-income}). 

%     \item Through numerical analysis, we demonstrate the efficiency of $\karma$ in reducing the bottleneck congestion. And show that it is very close to the theoretical efficiency attained by applying an optimal monetary tolling to  the fast lane (Section~\ref{sec:numerical-analysis}). 
    
%     \item \rev{We assess the robustness of $\karma$ to heterogeneous desired arrival times, demonstrating its ability to adapt to heterogeneous demands in a decentralized manner by simply introducing a karma cap (Section~\ref{subsec:heterogeneous-tstar}).}
%     % To be robust against small subpopulations that desire to arrive outside the congested period and therefore should not take part in the system, we propose the simple intervention of a karma cap beyond which commuters do not get redistributed more karma.
%     % We demonstrate that this successfully eliminates irrelevant users in a decentralized manner and without affecting the efficiency of the scheme;}

%     \item We showcase how the design degree of freedom represented by the karma redistribution can be exploited by policymakers. In fact, by considering a time-varying karma redistribution scheme further decongestion in the slow lane can be fostered (Section~\ref{sec:non-uniform-redistribution}).
%     \rev{With this scheme, $\karma$ outperforms the efficiency of an optimal monetary tolling scheme of the fast lane.}
% \end{itemize}

% We propose in Figure~\ref{fig:spdergraph} a qualitative representation of the different benefits and drawbacks of adopting different policies based on monetary tolling, tradable credits, or \karma. 
% \begin{figure}[H]
% \centering
% \includegraphics[trim={0 270 0 270},clip,frame,width=\textwidth]{figures/SpiderGraph.pdf}
% \caption{A qualitative depiction of the performances of: monetary tolling in (a),  tradable credits in (b), and \karma in (c). The considered features are: fairness for the commuters, privacy, and the effect in terms of traffic congestion alleviation.}
% \label{fig:spdergraph}
% \end{figure}


% \subsection{Notation}
% Let $a,d \in D\subseteq \Nat$  and let $c \in C\subseteq \Real^n$, then
% for a function $f : D \times C \rightarrow \Real$, we distinguish discrete and continuous arguments through the notation $f[d](c)$.
% Alternatively, we write $f : C \rightarrow \Real^{|D|}$ as the vector-valued function $f(c)$, with $f[d](c)$ denoting its $d^\textup{th}$ element.
% Similarly, $g[a \mid d](c)$ denotes the conditional probability of $a$ given $d$ and $c$. 
% Specifically, $g[d^+ \mid d](c)$ denotes one-step transition probabilities for $d$.
% We denote by $p \in \Delta(D):=\left\{\left. \sigma \in \Real_+^{|D|} \right\rvert \sum_{d \in D} \sigma[d] = 1 \right\}$ a probability distribution over the elements of $D$, with $p[d]$ denoting the probability of element $d$.
% Finally, when considering heterogeneous commuter types, we denote by $x_\tau$ a quantity associated to type $\tau$.

==> old_versions/model.tex <==
\section{CARMA: bottleneck congestion management with karma}
\label{sec:karma-bottleneck}
% Description of the karma mechanism on an high level. Hence the overall structure on how everything should work without to much math.
% Maybe good to add some schemes to better explain the setting.

We now specialize the general karma mechanism above to model the morning commute problem. 
We consider $N$ commuters that travel daily through a bottleneck.
The commuters are heterogeneous in their \rev{desired arrival times, as well as their} \emph{\gls{VOT} process}, that is, the process by which their daily \gls{VOT} multiplier $u$ changes.
\rev{For commuters of type $\tau$, we denote by $t^*_\tau$ their desired arrival time and by $\phi_\tau[u^+ \mid u]$ their VOT process.}
% Consider the $N$ commuters that repeatedly, e.g., every day, travel through a bottleneck, such as the one presented in Section~\ref{sec:bottleneck}. As anticipated in Section~\ref{sec:bottleneck}, we assume that the travelers might be  heterogeneous in their urgency processes $u$. 
We discretize the feasible departure times into $T$ intervals \rev{each of length $\Delta t$}. Therefore, on every morning, commuters with state $[u,k]$ make a decision on their departure time $t\in \T = \{1,\dots,T\}$ and bid to enter the fast lane $b\in\B[k]$.
% Those choosing a bid $b=0$ enter the slow lane by default.
Consequently, the highest $\sfast$ bidders departing at $t$ are allowed to enter the fast lane, while all others have to use the slow lane. The mechanism is illustrated in Figure~\ref{fig:karma_bottleneck}.

\begin{figure}[ht]
\includegraphics[width=\textwidth]{figures/karma-bottleneck.pdf}
\caption{Illustration of karma mechanism in bottleneck.}
\label{fig:karma_bottleneck}
\end{figure}

In what follows, we first specify the key model elements for $\karma$, i.e., the immediate reward and karma transition functions.
\rev{We then turn to a theoretical analysis of the $\karma$ \acrfull{SNE}, showing its existence as well as a strict Pareto improvement property with respect to no policy intervention.
This is followed by a comprehensive numerical analysis in Section~\ref{sec:numerical-analysis}.}

% We now specify the general karma dynamic population game presented in Section~\ref{sec:karma-preliminaries} to the bottleneck setting.
% There are $N$ travelers (with $N$ typically large) that must repeatedly traverse a bottleneck (e.g., every day).
% We consider that the travelers have heterogeneous urgency processes, as specified by their \emph{urgency type} $\tau$.
% This is loosely analogous to the heterogeneity in the value of time (VOT) in the classical bottleneck, a notion that will be made more precise hereafter.
% As in the general karma setting, each traveler has a state $(u,k) \in \U \times \Nat$ that varies every day.


% The urgency state evolves according to the exogenous type-dependent Markov chain $\phi_\tau[u^+ \mid u]$, independently for each traveler of that type.
% The bottleneck congestion occurs over a discrete time grid $\T = \{1,\dots,T\}$, with all the travelers having a common desired arrival time $t^* \in \T$\footnote{The model can readily incorporate heterogeneity in $t^*$ as a further type, which will be the subject of future work.}.
% The bottleneck has a total capacity of $S < N$ travelers per discrete time step, which is split into a \emph{fast lane} with capacity $S_1 < S$ and a \emph{slow lane} with capacity $S_2 = S - S_1$.
% In what follows, it will be convenient to express these capacities on a normalized scale. We let $s = \frac{S}{N}$, $s_1 = \frac{S_1}{N}$, and $s_2 = \frac{S_2}{N}$ be the total, slow lane, and fast lane normalized capacities, respectively, expressed as \emph{mass of travelers} per time step (a unit mass corresponds to the total amount of travelers $N$).
% Every day, each traveler must choose a \emph{departure time} $t \in \T$ at which to enter the bottleneck, as well as a \emph{karma bid} $b \in \B^k$ on entering the fast lane (the bid is limited by the karma $k$).
% Consequently, the traveler's \emph{action} is
% \[
%     a = (t,b) \in \A^k = \T \times \B^k.
% \]
% As in the general karma setting, the \emph{social state} $(d,\pi) \in \D \times \Pi$ consists of the type-state distribution $d$ (with $d_\tau[u,k]$ giving the mass of travelers in type $\tau$ and state $(u,k)$) and the policy $\pi$ (with $\pi_\tau[t,b \mid u,k]$ giving the probability of playing action $(t,b)$ by a traveler of type $\tau$ in state $(u,k)$).
% In order to complete the definition of the bottleneck karma dynamic population game, we now turn to specifying the \emph{immediate reward function}~\ref{eq:immediate-reward} and the \emph{karma transition function}~\ref{eq:karma-transition} in the bottleneck setting.

\subsection{Immediate reward function $\zeta_\rev{\tau}[u,t,b](d,\pi)$}
\label{subsec:immediate-reward}
Following the classical bottleneck model, we define the immediate reward in two parts: queuing delay $t^q$ and early or late schedule delay ($t^e_\rev{\tau}$ or $t^l_\rev{\tau}$, respectively). Given the departure time and bid, how much delay each commuter endures depends on the outcome of the karma auction. Let $\psi[o\mid t,b](d,\pi)$ denote the probability of an ego commuter finally entering lane $o\in\{\textup{fast},\textup{slow}\}$, given its choice of $t$, bid $b$ and the other commuters' actions (function of the social state $(d,\pi)$).
Then, the immediate reward can be written as
\begin{multline}
    \label{eq:bottleneck-immediate-reward}
    \zeta_\rev{\tau}[u,t,b](d,\pi) \\
    = - u \: \sum_o \psi[o \mid t,b](d,\pi) \left(\alpha \: t^q[t,o](d,\pi) + \beta \: t^e_\rev{\tau}[t,o](d,\pi) + \gamma \: t^l_\rev{\tau}[t,o](d,\pi) \right),
\end{multline}
where $t^q[t,o](d,\pi)$, $t^e_\rev{\tau}[t,o](d,\pi)$ and $t^l_\rev{\tau}[t,o](d,\pi)$ are given by
\begin{align}
    t^q[t,o](d,\pi) &= \begin{cases}
        0, & o=\textup{fast}, \\
        \frac{q[t](d,\pi)}{s_\textup{slow}}, & o=\textup{slow},
    \end{cases} \label{eq:queue-delay}\\
    t^e_\rev{\tau}[t,o](d,\pi) &= \max\{0, \; t^*_\rev{\tau} - t - t^q[t,o](d,\pi)\}, \\
    t^l_\rev{\tau}[t,o](d,\pi) &= \max\{0, \; t + t^q[t,o](d,\pi) - t^*_\rev{\tau}\}.
\end{align}
In Eq.~\ref{eq:queue-delay}, $q[t](d,\pi)$ gives the queue length on the slow lane at time $t$, i.e., it is the discrete-time equivalent of $q(t)$ defined in Section~\ref{sec:bottleneck}. Accordingly, if the commuter enters the fast lane, Eq.~\ref{eq:bottleneck-immediate-reward} reduces to  Eq.~\ref{eq:cost_fast_lane_bn} (negated for rewards instead of costs).
Otherwise, it reduces to Eq.~\ref{eq:cost_slow_lane_bn}.

To complete the definition of Eq.~\ref{eq:bottleneck-immediate-reward}, we now derive $\psi[o\mid t,b](d,\pi)$.
We define a threshold bid $b^*[t]$ such that 
\begin{itemize}
    \item if $b>b^*[t]$, the commuter enters the fast lane for sure, i.e., $o=\textup{fast}$;
    \item if $b<b^*[t]$, the commuter enters the slow lane for sure, i.e., $o=\textup{slow}$; 
     \item if $b=b^*[t]$, the commuter ties with others and enters the fast lane via a random draw on the remaining capacity.
\end{itemize}
Let $\nu[t,b](d,\pi)$ be the mass of commuters departing at $t$ and bidding $b$, i.e., 
\begin{align}
    \nu[t,b](d,\pi) = \sum_{\tau,u,k} d_\tau[u,k] \: \pi_\tau[t,b \mid u,k].
\end{align}
Then, $b^*[t]$ is given by 
\begin{align}\label{eq:b_star}
    b^*[t](d,\pi) = \max \left\{b\in\Nat \left| \: \sum_{b'\geq b} \nu [t,b'](d,\pi) \right.\geq \frac{s_\textup{fast}}{N}\right\}.
\end{align}
Accordingly, the probability of entering the fast lane is derived as 
\begin{align}
    \label{eq:prob-outcome}
    \psi[o = \textup{fast} \mid t,b](d,\pi) = \begin{cases}
    1, & b>b^*[t](d,\pi),\\
    0, & b<b^*[t](d,\pi),\\
    \frac{s_\textup{fast}/N - \sum_{b'>b}\nu[t,b'](d,\pi)}{\nu[t,b](d,\pi)}, & b=b^*[t](d,\pi),
    \end{cases}
\end{align}
\rev{and the probability of entering the slow lane is $\psi[o = \textup{slow} \mid t,b](d,\pi) = 1 - \psi[o = \textup{fast} \mid t,b](d,\pi)$.}




% Let $o \in \Out = \{1,2\}$ denote the karma auction \emph{outcome} to an ego traveler, with $o=1$ denoting that the traveler successfully enters the fast lane (and $o=2$ that the slow lane must be entered).
% This outcome will be a function of the ego traveler's own bid, how many other travelers are bidding to enter the fast lane at the same time, as well as those travelers' bids.
% Therefore, an important quantity is the \emph{distribution of actions} in the population.
% This can be readily derived from the social state as
% \begin{align}
%     \label{eq:action-dist}
%     \nu[t',b'](d,\pi) = \sum_{\tau,u,k} d_\tau[u,k] \, \pi_\tau[t',b' \mid u,k],
% \end{align}
% where $\nu[t',b'](d,\pi)$ denotes the mass of travelers departing at $t'$ and bidding $b'$ (we use $(t',b')$ to distinguish actions played by travelers other than the ego traveler).
% Conceptually, the outcome to an ego traveler departing at $t$ and bidding $b$ is determined by one of the following three cases:
% \begin{itemize}
%     \item \textbf{Win:} if the mass of travelers departing at $t'=t$ and bidding $b' \geq b$ is strictly smaller than $s_1$, the ego traveler is amongst the $s_1$ highest bidders and can surely enter the fast lane;
%     \item \textbf{Lose:} if the mass of travelers departing at $t'=t$ and bidding $b' > b$ meets or exceeds $s_1$, those travelers will fill the fast lane and there is no chance for the ego traveler to enter it.
%     \item \textbf{Tie:} if the mass of travelers departing at $t'=t$ and bidding $b' > b$ is strictly smaller than $s_1$ (and therefore those travelers surely enter the fast lane), but $s_1$ is met or exceeded once the mass of travelers bidding $b'=b$ is added, then the ego traveler is tied for the right to enter the fast lane with all other travelers bidding $b$.
%     In this case, the remaining capacity of the fast lane is filled by a subset of the tied travelers chosen uniformly at random.
% \end{itemize}
% Formally, this translates into the following \emph{probability to enter the fast lane}
% \begin{multline}
%     \label{eq:prob-outcome}
%     \psi[o = 1 \mid t,b](d,\pi) \\
%     = \begin{cases}
%         1, &\text{(win)\phantom{(lose)(tie)}\hspace{-40pt}if } \sum_{b' \geq b} \nu[t,b'](d,\pi) \leq s_1 - \epsilon, \\
%         0, &\text{(lose)\phantom{(win)(tie)}\hspace{-40pt}if } \sum_{b' > b} \nu[t,b'](d,\pi) \geq s_1, \\
%         \frac{s_1 - \sum_{b' > b} \nu[t,b'](d,\pi)}{\nu[t,b](d,\pi) + \epsilon}, &\text{(tie)\phantom{(win)(lose)}\hspace{-40pt}if } \sum_{b' > b} \nu[t,b'](d,\pi) < s_1 < \sum_{b' \geq b} \nu[t,b'](d,\pi) + \epsilon,
%     \end{cases}
% \end{multline}
% where we introduced a \emph{buffer parameter} $\epsilon > 0$ that can be made arbitrarily small.
% The probability of entering the slow lane is $\psi[o = 2 \mid t,b](d,\pi) = 1 - \psi[o = 1 \mid t,b](d,\pi)$.
% The parameter $\epsilon$ is needed to ensure the continuity of~\ref{eq:prob-outcome} in $(d,\pi)$, as we show next.




% \begin{proposition}
% \label{prop:outcome-continuous}
% For every $o \in \Out$, $(t,b) \in \T \times \Nat$, the outcome probability $\psi[o \mid t,b](d,\pi)$ is continuous at every $(d,\pi) \in \D \times \Pi$.
% \end{proposition}

% \begin{proof}
% Fix an arbitrary action $(t,b)$, and consider the probability of entering the fast lane $o=1$ (continuity for $o=2$ straightforwardly follows).
% Let $\nu \in \Delta(\T \times \Nat)$ be the vector formed by stacking $\nu[t',b']$ for all $(t',b') \in \T \times \Nat$.
% Note that we can write $\psi[o=1 \mid t,b](d,\pi)$ as $\psi[o=1 \mid t,b](\nu(d,\pi))$, i.e., the dependency of $\psi[o=1 \mid t,b]$ on $(d,\pi)$ is through $\nu(d,\pi)$.
% Since $\nu(d,\pi)$~\ref{eq:action-dist} is continuous at every $(d,\pi) \in \D \times \Pi$, it suffices then to show that $\psi[o=1 \mid t,b](\nu)$ is continuous at every $\nu \in \Delta(\T \times \Nat)$ (the composition of continuous functions is continuous).

% Let us decompose $\Delta(\T \times \Nat)$ into the following three sets
% \begin{align*}
%     \Vwin[t,b] &= \left\{\nu \in \Delta(\T \times \Nat) \left \lvert \; \sum_{b' \geq b} \nu[t,b'] \leq s_1 - \epsilon \right. \right\}, \\
%     \Vlose[t,b] &= \left\{\nu \in \Delta(\T \times \Nat) \left \lvert \; \sum_{b' > b} \nu[t,b'] \geq s_1 \right. \right\}, \\
%     \Vtie[t,b] &= \left\{\nu \in \Delta(\T \times \Nat) \left \lvert \; \sum_{b' > b} \nu[t,b'] < s_1 < \sum_{b' \geq b} \nu[t,b'] + \epsilon \right. \right\}.
% \end{align*}
% It is straightforward to verify that these sets are disjoint and that $\Vwin[t,b] \cup \Vlose[t,b] \cup \Vtie[t,b] = \Delta(\T \times \Nat)$.
% Continuity of~\ref{eq:prob-outcome} straightforwardly holds at every $\nu$ in the interior of $\Vwin[t,b]$ and the interior of $\Vlose[t,b]$ ($\psi[o=1 \mid t,b](\nu)$ is constant), as well as at every $\nu \in \Vtie[t,b]$ (guaranteed by the parameter $\epsilon > 0$).
% Therefore, a discontinuity can only occur at the boundary of $\Vwin[t,b]$ or the boundary of $\Vlose[t,b]$.

% For an arbitrary $\nu^\textup{win}$ on the boundary of $\Vwin[t,b]$, i.e., satisfying $\sum_{b' \geq b} \nu^\textup{win}[t,b'] = s_1 - \epsilon$, and a $\nu' \rightarrow \nu^\textup{win}$, it either holds that
% \begin{align*}
%     \lim_{\sum_{b' \geq b} \nu'[t,b'] \rightarrow (s_1 - \epsilon)^-} \psi[o-1 \mid t,b](\nu') = \lim_{\sum_{b' \geq b} \nu'[t,b'] \rightarrow s_1 - \epsilon} \psi[o-1 \mid t,b](\nu') = 1 \quad (\nu' \in \Vwin[t,b]),
% \end{align*}
% or it holds that
% \begin{multline*}
%     \lim_{\sum_{b' \geq b} \nu'[t,b'] \rightarrow (s_1 - \epsilon)^+} \psi[o-1 \mid t,b](\nu') = \lim_{\sum_{b' \geq b} \nu'[t,b'] \rightarrow (s_1 + \epsilon)^+} \frac{s_1 - \sum_{b' \geq b} \nu'[t,b'] + \nu'[t,b]}{\nu'[t,b] + \epsilon} \\
%     = \frac{\nu'[t,b] + \epsilon}{\nu'[t,b] + \epsilon} = 1  \quad (\nu' \in \Vtie[t,b]).
% \end{multline*}
% Note that a $\nu'$ sufficiently close to $\nu^\textup{win}$ cannot lie in $\Vlose[t,b]$, since
% \begin{multline*}
%     \sum_{b' \geq b} \nu^\textup{win}[t,b'] = s_1 - \epsilon \Rightarrow \sum_{b' \geq b} \nu^\textup{win}[t,b'] < s_1 \Rightarrow \sum_{b' > b} \nu^\textup{win}[t,b'] < s_1 \\
%     \Rightarrow \sum_{b' > b} \nu'[t,b'] < s_1 \text{ for } \nu' \rightarrow \nu^\textup{win}.
% \end{multline*}
% This proves that $\psi[o-1 \mid t,b](\nu)$ is continuous at $\nu^\textup{win}$.

% The continuity of $\psi[o=1 \mid t,b](\nu)$ at every $\nu^\textup{lose}$ on the boundary of $\Vlose[t,b]$ (i.e., satisfying $\sum_{b' > b} \nu^\textup{lose}[t,b'] = s_1$) follows similar arguments which are omitted for brevity.
% We can hence conclude that $\psi[o=1 \mid t,b](\nu)$ is continuous at every $\nu \in \Delta(\T \times \Nat)$.
% \end{proof}


% \blue{We can now derive the mass of commuters entering each lane at time $t$ as}
% % We can now proceed with deriving the mass of agents departing at the fast ($o=1$) and the slow ($o=2$) lanes at every time step, as 
% \begin{align}
%     \label{eq:departures}
%     n[t,o](d,\pi) = \sum_b \nu[t,b](d,\pi) \: \psi[o \mid t,b](d,\pi).
% \end{align}
% With  ~\ref{eq:prob-outcome-cont}, we can show the fast lane is never congested. This result is formally stated in the following propostion. 
% % By the design of $\psi[o=1 \mid t,b](d,\pi)$~\ref{eq:prob-outcome}, the fast lane is never congested, as we show next.
% \red{\begin{proposition}
% For all $t \in \T$, $(d,\pi) \in \D \times \Pi$, it holds that $n[t,o=\textup{fast}](d,\pi) < s_\textup{fast}/N$. \red{or $\leq$?}
% \end{proposition}
% \begin{proof}
% \todo{Write proof}
% \end{proof} }



% It follows that the fast lane never experiences a queue, i.e., it always holds that $q[t,o=1](d,\pi)=0$.
% On the other hand, the queue in the slow lane is given by
% \begin{align*}
%     q[t=1,o=2](d,\pi) &= \max\{0, \; n[t=1,o=2](d,\pi) - s_2\}, \\
%     q[t,o=2](d,\pi) &= \max\{0, \; q[t-1,o=2](d,\pi) + n[t,o=2](d,\pi) - s_2\}, \quad \forall t > 1.
% \end{align*}
% Note that, since the point-wise maximum of continuous functions is continuous, it holds that $q[t=1,o=2](d,\pi)$ is continuous in $(d,\pi)$ (using the continuity of $n[t=1,o=2](d,\pi)$~\ref{eq:departures}).
% Using an inductive argument, it is straightforward to show that $q[t,o=2](d,\pi)$ is continuous for all $t > 1$ as well.

% With this, we can derive the expected \emph{queuing delay} $t^q[t,o](d,\pi)$, \emph{schedule early delay} $t^e[t,o](d,\pi)$, and \emph{schedule late delay} $t^l[t,o](d,\pi)$ for a traveler departing at time $t$ and entering lane $o$.
% \begin{align*}
%     t^q[t,o](d,\pi) &= \begin{cases}
%         0, &\text{if } o=1, \\
%         \frac{q[t,o](d,\pi)}{s_2}, &\text{if } o=2.
%     \end{cases}, \\
%     t^e[t,o](d,\pi) &= \max\{0, t^* - t - t^q[t,o](d,\pi)\}, \\
%     t^l[t,o](d,\pi) &= \max\{0, t + t^q[t,o](d,\pi) - t^*\}.
% \end{align*}
% Note that they are all continuous in $(d,\pi)$.

% Finally, the immediate reward function $\zeta[u,t,b](d,\pi)$ in the bottleneck karma game is
% \begin{align}
%     \label{eq:bottleneck-immediate-reward}
%     \zeta[u,t,b](d,\pi) = u \: \sum_o \psi[o \mid t,b](d,\pi) \left(\alpha \: t^q[t,o](d,\pi) + \beta \: t^e[t,o](d,\pi) + \gamma \: t^l[t,o](d,\pi) \right),
% \end{align}
% where $\beta < \alpha < \gamma$ are the schedule early, queuing, and schedule late delay penalty parameters, respectively.
% Note that is is also continuous in $(d,\pi)$

\subsection{Karma transition function $\kappa[k^+ \mid k,t,b](d,\pi)$}
\label{subsec:karma-transition}

The karma transition function encodes the rules of how karma is transferred between the commuters.
There are significant degrees of freedom in the design of these rules.
\rev{For the sake of presentation we showcase here a simple scheme, and dedicate Section~\ref{sec:non-uniform-redistribution} to the exploration of more elaborate designs.}
% , though in this work we opt for a simple scheme.
% The experimentation of different schemes is an interesting extension that is left for future works.
All commuters entering the fast lane pay their bids, and at the end of each day, the total payments are uniformly redistributed to all commuters in the system (including those who entered the fast lane).
Formally, similarly to Eq.~\ref{eq:cost_fast_lane_bn}, let $p[b,o]$ be the karma payment made by a commuter who bids $b$ and enters lane $o$, then we have 
\begin{align}
    \label{eq:payment}
    p[b,o] = \begin{cases}
        b, & o=\textup{fast}, \\
        0, & o=\textup{slow}.
    \end{cases}
\end{align}
Accordingly, the \emph{average payment} is computed by aggregating Eq.~\ref{eq:payment} over all commuters, i.e.,
\begin{multline}
    \pbar(d,\pi) = \sum_{t,b} \nu[t,b](d,\pi) \sum_o \psi[o \mid t,b](d,\pi) \: p[b,o] \\
    = \sum_{t,b} \nu[t,b](d,\pi) \: \psi[o=\text{fast} \mid t,b](d,\pi) \: b. \label{eq:average-payment}
\end{multline}
To preserve the integer value of karma, $\ceil{\pbar(d,\pi)}$ is randomly distributed to some commuters and $\floor{\pbar(d,\pi)}$ to the others. Specifically, the mass of commuters receiving $\ceil{\pbar(d,\pi)}$ units of karma is given by $f(d,\pi) = \pbar(d,\pi) - \floor{\pbar(d,\pi)}$.
% This gets redistributed to all the travelers using the following integer-preserving scheme:
% \begin{itemize}
%     \item distribute $\floor{\pbar(d,\pi)}$ to a mass $f^\textup{low}(d,\pi)=\ceil{\pbar(d,\pi)} - \pbar(d,\pi)$ of travelers, randomly selected;
%     \item distribute $\ceil{\pbar(d,\pi)}$ to the remaining mass $f^\textup{high}(d,\pi)= 1 - f^\textup{low}(d,\pi)$ of travelers.
% \end{itemize}
% Consequently, the probability that an ego traveler receives a redistribution of $\floor{\pbar(d,\pi)}$ (respectively, $\ceil{\pbar(d,\pi)}$) is $f^\textup{low}(d,\pi)$ (respectively, $f^\textup{high}(d,\pi)$).
This yields the following karma transition probabilities, conditional on the outcome $o$:
\begin{align}
    \label{eq:bottleneck-karma-tranistions-o}
    \Prob[k^+ \mid k,t,b,o](d,\pi) = \begin{cases}
        f(d,\pi), & o = \textup{fast}, \text{ and } k^+ = k - b + \ceil{\pbar(d,\pi)}, \\
        1-f(d,\pi), & o =  \textup{fast}, \text{ and } k^+ = k - b + \floor{\pbar(d,\pi)}, \\
        f(d,\pi), & o =  \textup{slow}, \text{ and } k^+ = k + \ceil{\pbar(d,\pi)}, \\
        1-f(d,\pi), & o =  \textup{slow}, \text{ and } k^+ = k + \floor{\pbar(d,\pi)}, \\
        0, &\text{otherwise}.
    \end{cases}
\end{align}
% \begin{align}
%     \label{eq:bottleneck-karma-tranistions-o}
%     \Prob[k^+ \mid k,t,b,o](d,\pi) = \begin{cases}
%         f^\textup{low}(d,\pi), &\text{if } o = 1 \text{ and } k^+ = k - b + \floor{\pbar(d,\pi)}, \\
%         f^\textup{high}(d,\pi), &\text{if } o = 1 \text{ and } k^+ = k - b + \ceil{\pbar(d,\pi)}, \\
%         f^\textup{low}(d,\pi), &\text{if } o = 2 \text{ and } k^+ = k + \floor{\pbar(d,\pi)}, \\
%         f^\textup{high}(d,\pi), &\text{if } o = 2 \text{ and } k^+ = k + \ceil{\pbar(d,\pi)}, \\
%         0, &\text{otherwise}.
%     \end{cases}
% \end{align}
Note that Eq.~\ref{eq:bottleneck-karma-tranistions-o} does not explicitly depend on the departure time $t$, but we write a dependency here for generality.
\rev{We will consider time-dependant redistribution schemes in Section~\ref{sec:non-uniform-redistribution}.}
% It is straightforward to verify that Eq.~\ref{eq:bottleneck-karma-tranistions-o} is continuous in $(d,\pi)$.
Finally, we can construct the karma transition function as
\begin{align}
    \label{eq:bottleneck-karma-transitions}
    \kappa[k^+ \mid k,t,b](d,\pi) = \sum_o \psi[o \mid t,b](d,\pi) \: \Prob[k^+ \mid k,t,b,o](d,\pi).
\end{align}

\rev{
\subsection{\acrfull{SNE} analysis}
We now perform a theoretical analysis of the $\karma$ \gls{SNE}, showing its existence as well as that it leads to a strict Pareto improvement of all commuter types with respect to no policy intervention.
The theoretical analysis is complemented by a comprehensive numerical analysis in Section~\ref{sec:numerical-analysis}.

\subsubsection{Existence of \gls{SNE}}
We verify that $\karma$ satisfies Assumptions~\ref{as:continuity} and~\ref{as:karma-preservation}, needed to guarantee the existence of a \gls{SNE} (Theorem~\ref{th:Nash-exists}).

\paragraph{Assumption~\ref{as:continuity} (Continuity)}
It is straightforward to verify that all the expressions in the derivation of $\zeta_\tau[u,t,b](d,\pi)$ and $\kappa[k^+ \mid k,t,b](d,\pi)$ are continuous in $(d,\pi)$, with the exception of $\psi[o = \textup{fast} \mid t,b](d,\pi)$ (Eq.~\ref{eq:prob-outcome}) which has a discontinuity at $\nu[t,b](d,\pi)=0$.
% Note that $\psi[o = \textup{fast} \mid t,b](d,\pi)$ is continuous in $(d,\pi)$ except where $\nu[t,b](d,\pi)=0$.
% To ensure that Assumption~\ref{as:continuity} is satisfied,
Therefore,} we approximate Eq.~\ref{eq:prob-outcome} with a function that is continuous everywhere, given by
\begin{multline}
    \label{eq:prob-outcome-cont}
    \psi^\epsilon[o = \textup{fast} \mid t,b](d,\pi) \\
    = \begin{cases}
    1, & \sum_{b'> b} \nu[t,b'](d,\pi)\leq \frac{s_\textup{fast}}{N} -  \nu[t,b](d,\pi) -\epsilon, \\
    0, & \sum_{b'> b} \nu[t,b](d,\pi)\geq \frac{s_\textup{fast}}{N}, \\
    \frac{s_\textup{fast}/N-\sum_{b'>b}\nu[t,b](d,\pi)}{\nu[t,b](d,\pi)+\epsilon}, & \frac{s_\textup{fast}}{N} -  \nu[t,b](d,\pi) - \epsilon <  \sum_{b'> b} \nu[t,b'](d,\pi) < \frac{s_\textup{fast}}{N},
    \end{cases}
\end{multline}
where $\epsilon>0$ is an approximation parameter.
A graphic illustration is shown in Figure~\ref{fig:prob-outcome}, demonstrating the continuity of $\psi^\epsilon$ and that $\psi^\epsilon \rightarrow \psi$ as $\epsilon \rightarrow 0$.
\rev{The approximation parameter $\epsilon$ slightly under-allocates the fast lane: the commuters tying at the threshold bid $b^*[t]$ enter a random draw on the remaining capacity with a mass of $\nu[t,b^*[t]](d,\pi) + \epsilon$ rather than $\nu[t,b^*[t]](d,\pi)$ commuters.
In other words, $\epsilon$ can be interpreted as a `fictitious' mass of commuters bidding $b^*[t]$ and therefore slightly decreasing the chances of `real' commuters to enter the fast lane.
Since $\epsilon$ can be made arbitrarily small, using $\psi^\epsilon[o \mid t,b](d,\pi)$ instead of $\psi[o \mid t,b](d,\pi)$ guarantees that Assumption~\ref{as:continuity} holds with a negligible effect on the $\karma$ allocation.
}

\begin{figure}[ht]
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/prob-outcome-1.pdf}
\caption{$\nu[t,b](d,\pi)>0$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/prob-outcome-2.pdf}
\caption{$\nu[t,b](d,\pi)=0$}
\end{subfigure}
\caption{Illustration of the exact and approximate outcome probability.
% $(d,\pi)$ is omitted for the simplicity of notation.
}
\label{fig:prob-outcome}
\end{figure}

% Clearly, Eq.~\ref{eq:bottleneck-karma-transitions} is also continuous in $(d,\pi)$.
% The following result ensures that Assumption~\ref{as:karma-preservation}, necessary to invoke  Theorem~\ref{th:Nash-exists}, also holds.

\rev{
\paragraph{Assumption~\ref{as:karma-preservation} (Karma preservation)} It is straightforward to verify that the considered karma transition scheme is karma preserving, as is shown in Proposition~\ref{prop:karma-preservation}.
}
\begin{proposition}
\label{prop:karma-preservation}
The karma transition function Eq.~\ref{eq:bottleneck-karma-transitions} satisfies Assumption~\ref{as:karma-preservation}, i.e., karma is preserved in expectation.
\end{proposition}

\begin{proof}
We verify that condition Eq.~\ref{eq:karma-preservation} is satisfied as follows (the dependency on $(d,\pi)$ is omitted in the notation):
\begin{align*}
    &\sum_{\tau,u,k} d_\tau[u,k] \sum_{t,b} \pi_\tau[t,b \mid u,k] \sum_{k^+} \kappa[k^+ \mid k,t,b] \: k^+ \\
    &\quad=\sum_{\tau,u,k} d_\tau[u,k] \sum_{t,b} \pi_\tau[t,b \mid u,k] \sum_o \psi[o \mid t,b] \sum_{k^+} \Prob[k^+ \mid k,t,b,o] \: k^+ \\
    % &\quad= \sum_{\tau,u,k} d_\tau[u,k] \sum_{t,b} \pi[t,b \mid u,k] \left(\psi[o=1 \mid t,b] \: (k - b + \pbar) + \psi[o=2 \mid t,b] \: (k + \pbar) \right) \\
    &\quad= \sum_{\tau,u,k} d_\tau[u,k] \sum_{t,b} \pi_\tau[t,b \mid u,k] \left(\psi[o=\textup{fast} \mid t,b] \: (k - b + \pbar) \right. \\
    &\quad\phantom{= \sum_{\tau,u,k} d_\tau[u,k] \sum_{t,b} \pi_\tau[t,b \mid u,k]}\qquad \left. + \psi[o=\textup{slow} \mid t,b] \: (k + \pbar) \right)\\
    &\quad= \sum_{\tau,u,k} d_\tau[u,k] \: k + \pbar - \sum_{\tau,u,k} d_\tau[u,k] \sum_{t,b} \pi_\tau[t,b \mid u,k] \: \psi[o=\text{fast} \mid t, b] \: b \\
    &\quad= \sum_{\tau,u,k} d_\tau[u,k] \: k.
\end{align*}
The equality from the second to the third line is due to $(1-f)\floor{\pbar} + f\ceil{\pbar}=\pbar$. 
%where we use $f^\textup{low}\: \floor{\pbar} + f^\textup{high} \: \ceil{\pbar} = \pbar$.
\end{proof}

% Given Proposition~\ref{prop:karma-preservation} and the continuity of the immediate reward  Eq.~\ref{eq:bottleneck-immediate-reward} and karma transition  Eq.~\ref{eq:bottleneck-karma-transitions}, the karma mechanism for the bottleneck model is well-posed, i.e., 
\rev{Putting everything together, using $\psi^\epsilon[o \mid t,b](d,\pi)$ guarantees the existence of a $\karma$ \gls{SNE} and the well-posedness of the $\karma$ scheme.} The equilibrium can be computed using an evolutionary dynamics~\cite{sandholm2010population} inspired algorithm, as described in detail in \cite{elokda2022self}~Algorithm 1.
% Using Proposition~\ref{prop:karma-preservation} and the continuity of $\zeta[u,t,b](d,\pi)$~\ref{eq:bottleneck-immediate-reward} and $\kappa[k^+ \mid k,t,b](d,\pi)$~\ref{eq:bottleneck-immediate-reward} in the social state $(d,\pi)$ (consequence of Proposition~\ref{prop:outcome-continuous}), the bottleneck karma dynamic population game is well-posed, i.e., a stationary Nash equilibrium is guaranteed to exist in this game (Theorem~\ref{th:Nash-exists}).

\subsubsection{Strict Pareto improvement with respect to no policy intervention}
\label{subsubsec:pareto-improvement}

In this section, we assume that all commuters desire to arrive during the congested period, i.e., $t^*_\tau \in (\tstart,\tend)$ for all $\tau$, where $\tstart$ and $\tend$ are as given in Eq.~\ref{eq:tstart-tend-tpeak}.
Without loss of generality, we further assume that the congested period coincides with the discrete time interval $\T$ and that the desired arrival times $t^*_\tau$ coincide with discrete time steps in $\T$, i.e., it holds that $\frac{\tstart}{\Delta t} + 1 = 1$,
% $1 = \tstart \: \Delta t + 1$,
$\frac{\tend}{\Delta t} + 1 = T$, and $\frac{t^*_\tau}{\Delta t} + 1 \in \T$ for all $\tau$.

\begin{proposition}
\label{prop:karma-fast-lane}
In a $\karma$ \gls{SNE} $(d^*,\pi^*)$, all commuter types $\tau$ have a non-zero stationary probability of entering the fast lane.
\end{proposition}

\begin{proof}
Assume, for the sake of contradiction, that commuters of an arbitrary type $\tau$ never enter the fast lane in a \gls{SNE} $(d^*,\pi^*)$.
This means that the equilibrium policy $\pi_\tau^*$ places zero weight on any bid for which the commuter can enter the fast lane, i.e.,
\begin{align}
\forall [u,k] \in \X : d_\tau^*[u,k] > 0, \; \forall t \in \T, \; \forall b \geq b^*[t](d^*,\pi^*), \quad \pi_\tau^*[t,b \mid u,k] = 0. 
\end{align}
Since the slow lane experiences congestion, the type $\tau$ commuter will always experience a non-zero immediate travel cost.
Moreover, since the commuter never uses karma to enter the fast lane, the immediate cost is a function of the urgency only and not the karma. It follows that
\begin{align*}
R_\tau[u,k](d^*,\pi^*) &= R_\tau[u](d^*,\pi^*) < 0, \\
V_\tau[u,k](d^*,\pi^*) &= V_\tau[u](d^*,\pi^*) = R_\tau[u](d^*,\pi^*) + \delta \sum_{u^+} \phi_\tau[u^+ \mid u] \: V_\tau[u^+](d^*,\pi^*) \\
&\qquad < \delta \sum_{u^+} \phi_\tau[u^+ \mid u] \: V_\tau[u^+](d^*,\pi^*).
\end{align*}
The type $\tau$ commuter never pays karma since they never enter the fast lane.
Every day, however, they receive a karma redistribution of at least $\floor{\pbar(d^*,\pi^*)}$.
Therefore, after a maximum of $\frac{b^*_\tau[t^*](d^*,\pi^*) + 1}{\floor{\pbar(d^*,\pi^*)}}$ days, they will have accumulated at least karma $k > b^*[t^*_\tau](d^*,\pi^*)$.
It follows that there is a state $[\tilde u,\tilde k]$ with $\tilde k > b^*[t^*_\tau](d^*,\pi^*)$ for which $d^*_\tau[\tilde u, \tilde k] > 0$.
Let us consider the single-stage deviation reward for deviating from $\pi_\tau^*$ to play $[\tilde t, \tilde b] = [t^*_\tau,b^*[t^*_\tau](d^*,\pi^*) + 1]$ when in state $[\tilde u,\tilde k]$,
\begin{align*}
Q_\tau[\tilde u, \tilde k, \tilde t, \tilde b](d^*,\pi^*) &= \zeta[\tilde u, \tilde t, \tilde b](d^*,\pi^*) \\
&\quad + \delta \: \sum_{u^+,k^+} \phi_\tau[u^+ \mid \tilde u] \: \kappa[k^+ \mid \tilde k, \tilde t, \tilde b](d^*,\pi^*) \: V_\tau[u^+,k^+](d^*,\pi^*) \\
&= 0 + \delta \: \sum_{u^+} \phi_\tau[u^+ \mid \tilde u] \: V_\tau[u^+](d^*,\pi^*) \\
&> V_\tau[\tilde u, \tilde k](d^*,\pi^*).
\end{align*}
Therefore, the type $\tau$ commuter has an incentive to deviate from $\pi^*_\tau$ and enter the fast lane when in state $[\tilde u,\tilde k]$.
This contradicts that $\pi^*_\tau$ is a \gls{SNE} policy (Eq.~\ref{eq:SNE-2}), concluding the proof.
\end{proof}

The proof of Proposition~\ref{prop:karma-fast-lane} formalizes the intuitive notion that if a commuter does not get to enter the fast lane, they will eventually collect enough karma to guarantee that they can, which is in their rational best interest.
In other words, the only possibility that a commuter never enters the fast lane is if they irrationally spare karma indefinitely.
Therefore, with $\karma$ any rational commuter has a non-zero stationary probability of entering the fast lane.
This has the following consequences.

\begin{corollary}
\label{cor:pareto-improvement}
In a $\karma$ \gls{SNE}, all commuter types $\tau$ experience a strict Pareto average travel cost improvement with respect to no policy intervention.
\end{corollary}

\begin{corollary}
For all commuter types $\tau$, there is a strict incentive to participate in the $\karma$ scheme as opposed to always using the slow lane.
\end{corollary}

\begin{proof}
From classical results, it is well known that the normalized equilibrium travel cost with no policy intervention equals the normalized equilibrium travel cost for using the slow lane $c^*_\tau$ (given in Eq~\ref{eq:classical-equilibrium-cost}) when the fast lane is occupied at the free-flow capacity.
Moreover, $c^*_\tau$ is a strict upper bound for the normalized travel cost of using the fast lane\footnote{\rev{with the exception of at the edge points $t=\tstart_\tau$ and $t=\tend_\tau$, it is rather annoying to deal with these edge cases}}.
Therefore, the only possibility for a commuter to not experience a strict Pareto improvement with respect to no policy intervention, or to not have a strict incentive to participate in $\karma$, is if the commuter never enters the fast lane.
Proposition~\ref{prop:karma-fast-lane} guarantees that entering the fast lane is always possible under $\karma$.
\end{proof}

As we will demonstrate in the upcoming numerical analysis, this stands in sharp contrast to classical monetary tolling policies under which some commuter types might not experience any benefit.

==> old_versions/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\subsection{Bottleneck model with lane segmentation}\label{sec:bottleneck}
To formalize $\karma$, we first recast a classical analysis framework for the morning commute problem~\cite{edara2008model} that is suitable to the karma mechanism.  

\tbc{Consider a bottleneck with $N$ commuters passing a single bottleneck with capacity $s$. The bottleneck is split into two lanes: a fast lane with capacity $\sfast$ that is tolled to be free of congestion, and a regular (or slow) lane with capacity $\sslow$ that is subject to congestion. }

Assume commuters are heterogeneous in their \gls{VOT} and desired arrival time. Specifically, they are classified into a finite number of groups and those from group $\tau$ share the same desired arrival time $t^*_\tau$. Following \cite{vickrey1973pricing} and \cite{xiao2013managing}, we assume commuters share the same ratio of queuing penalty over early/late arrival penalty, but differ in their urgency levels, denoted as $u$. Let $\alpha$, $\beta$, $\gamma$ be the normalized queuing, early arrival, and late arrival penalty, respectively. 

% Consider a bottleneck with $N$ commuters sharing the same desired arrival time $t^*$ \rev{(TODO: generalize to heterogeneous $t^*_\tau$)} and experiencing a single source of congestion identified by the bottleneck capacity $s$.
% The bottleneck is split into two lanes: the fast lane with capacity $\sfast$ is tolled and free of congestion, while the regular (or slow) lane with capacity $\sslow$ is subject to congestion. 
% Let $\alpha$, $\beta$, $\gamma$ be the normalized queuing, early arrival, and late arrival penalty, respectively. As in~\cite{vickrey1973pricing} and \cite{xiao2013managing}, we assume  that commuters are heterogeneous in their \gls{VOT} but share the same ratios of queuing penalty over early/late arrival penalty, i.e., $\frac{\alpha}{\beta}$ and $\frac{\alpha}{\gamma}$. This setup can be modeled by classifying the commuters into $M$ groups. Each group $j\in\{ 1,\dots,M \}$ is associated with a multiplier $u_j$ describing their \gls{VOT}, and without loss of generality we consider that $u_1<\dots<u_M$.
% % and  a fraction $h_j\in[0,1]$ that satisfies $\sum_{j=1}^Mh_j=1$ that identifies the percentage of the total vehicles in group $j$.} 
% %In this study, we consider travelers are classified into $M$ groups, each with a multiplier $u_j$ and fraction $p_j$. 
% % Suppose groups are ordered such that $u_1<u_2<\dots<u_M$. 
Then, the \emph{travel cost} for commuters who enter the fast lane at $t$ reads
\begin{align}
\label{eq:cost_fast_lane_bn}
    \cfast_\rev \tau[u](t) = \begin{cases}
    u \: \beta \: (t^*_\rev \tau-t), & t\leq t^*_\rev \tau, \\
     u \: \gamma \: (t-t^*_\rev \tau), & t>t^*_\rev \tau,
  \end{cases}
\end{align} 
and their total cost is given by $\hat c^\textup{fast}_\tau[u](t)= c^\textup{fast}_\tau[u](t)+p(t)$, where $p(t)$ is the toll price at time $t$.
If these commuters travel via the slow lane, their cost is 
\begin{align}
\label{eq:cost_slow_lane_bn}
 \cslow_\rev \tau[u](t) = \begin{cases}
     u \left[\alpha \: \frac{q(t)}{\sslow} + \beta \: (t^*_\rev \tau - t - \frac{q(t)}{\sslow}) \right], & t + \frac{q(t)}{\sslow}\leq t^*_\rev \tau, \\
     u \left[\alpha \: \frac{q(t)}{\sslow} + \gamma \: (t + \frac{q(t)}{\sslow} - t^*_\rev \tau) \right], & t + \frac{q(t)}{\sslow}>t^*_\rev \tau,
 \end{cases}
\end{align}
where $q(t)$ denotes the queue length on the slow lane at time $t$. 

\kz{
For commuters entering the slow lane, the equilibrium condition states that 
\begin{align}\label{eq:eq-slow-lane}
    \rev{r_\tau[u](t) > 0 \Rightarrow \;} 0\equiv \frac{\partial c^\textup{slow}_\tau[u](t)}{\partial t} = 
    \begin{cases}
    \frac{u}{\sslow}\left[\alpha q'(t) -\beta \left(1+\sslow\right)q'(t)\right], & t + \frac{q(t)}{\sslow}\leq t^*_\tau, \\
    \frac{u}{\sslow} \left[\alpha q'(t) + \gamma \left(1+\sslow\right)q'(t)\right], & t + \frac{q(t)}{\sslow}>t^*_\tau,
    \end{cases}
\end{align}
which yields
\begin{align}\label{eq:eq-queue-derv}
    \rev{r_\tau[u](t) > 0 \Rightarrow \;} q'(t) = 
    \begin{cases}
        \frac{\beta}{\alpha-\beta} \: \sslow, & t + \frac{q(t)}{\sslow}\leq t^*_\tau, \\
        -\frac{\gamma}{\alpha+\gamma} \: \sslow, & t + \frac{q(t)}{\sslow}>t^*_\tau.
    \end{cases}
\end{align}
\rev{\emph{EE: I think Eq.~\ref{eq:eq-slow-lane}--\ref{eq:eq-toll-derve} were missing that these conditions have to hold only if the $[\tau,u]$ commuters are putting positive weight on departing at time $t$; that is why I added the $r_\tau[u](t) > 0$ term (for departure rate).}} Eq.~\eqref{eq:eq-queue-derv} implies that, regardless of the urgency level, the queue length observed by commuters in group $\tau$ increases linearly at rate $\beta/(\alpha-\beta)$ if they arrive before $t^*_\tau$ and decreases linearly at rate $\gamma/(\alpha+\gamma)$ if they arrive after $t^*_\tau$. 

As suggested by \cite{arnott1988schedule}, with heterogeneous desired arrival time, the bottleneck could exhibit a single peak (when there is a dominant group or the desired arrival times are close) or multiple peaks (when groups have comparable sizes but quite different desired arrival times). With Eq.~\eqref{eq:eq-queue-derv}, it can be concluded that, in the case of single-peak, all commuters from the dominated group arrive either earlier or later than their desired arrival time, and their departures are mixed with those from the dominant group. On the other hand, when there exist multiple peaks, commuter groups have disjoint departure windows. It is also worth noting that, within each commuter group, the departure time is independent of the urgency level. 

Similarly, we can derive the optimal toll price on the fast lane using the equilibrium condition
\begin{align}
\label{eq:eq-toll-derve}
    \rev{r_\tau[u](t) > 0 \Rightarrow \;} 0\equiv \frac{\partial \hat{c}^\textup{fast}_\tau[u](t)}{\partial t} = 
    \begin{cases}
        -u\beta + p'(t), & t\leq t^*_\tau,\\
        u\gamma + p'(t), & t> t^*_\tau,
    \end{cases}
\end{align}
Accordingly, the tolling scheme is piece-wise linear and commuters with higher urgency will depart closer to their desired arrival times. This result is in line with previous studies on heterogeneous VOT (e.g., \cite{arnott1988schedule,liu2011morning}). 
The correspondence between the slow and fast lanes is established such that the toll price on the fast lane is equal to the queuing cost if the commuters switch to the slow lane~\cite{newell1987morning}. Figure~\ref{fig:model} gives an illustration of two commuter groups in different scenarios discussed above. 


In the scenarios of single-peak with two commuter groups shown in Figures~\ref{fig:model}(a) and (b), the starting and ending times of the peak hours ($\tstart$ and $\tend$), as well as the time with maximum queuing delay ($\tpeak$), can be derived respectively as follows~\cite{sun:2020:managing_bn_incentives}:
\begin{align}
    \label{eq:tstart-tend-tpeak}
    \tstart = t^*_{\tau_1}-c^*/\beta,\quad \tend = t^*_{\tau_1} +c^*/\gamma,\quad \tpeak = t^*_{\tau_1} - c^*/\alpha,
\end{align}
where $t^*_{\tau_1}$ is the desired arrival time of the dominant commuter group $\tau_1$ and   
\begin{align}
\label{eq:classical-equilibrium-cost}
c^* = \frac{\beta\gamma}{\beta+\gamma} \: \frac{N}{s}
\end{align}
is the corresponding normalized equilibrium cost. In other words, the equilibrium cost for each commuter in group $\tau_1$ with urgency $u$ is $u \: c^*$.

According to the relationship between $t^*_{\tau_1}$ and $t^*_{\tau_2}$, we can further derive the normalized equilibrium cost of group $A$ as
\begin{align}
    c^*_{\tau_2} = 
    \begin{cases}
        c^* - \beta(t^*_{\tau_1}-t^*_{\tau_2}), & t^*_{\tau_2}< t^*_{\tau_1},\\
        c^* - \gamma(t^*_{\tau_2}-t^*_{\tau_1}), & t^*_{\tau_2} > t^*_{\tau_1},
    \end{cases}
\end{align}

\begin{figure}[H]
\begin{subfigure}{0.95\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/model_eq_hetero_c1.pdf}
\caption{A dominated group with early desired arrival time and low VOT.}
\end{subfigure}
\begin{subfigure}{0.95\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/model_eq_hetero_c2.pdf}
\caption{A dominated group with late desired arrival time and high VOT.}
\end{subfigure}
\begin{subfigure}{0.95\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/model_eq_hetero_c3.pdf}
\caption{Two comparable groups with disjoint departure windows.}
\end{subfigure}
\caption{Illustration of bottleneck equilibrium with heterogeneous commuters (left: departures/arrivals on slow lane; right: optimal toll price on fast lane).}
\label{fig:model}
\end{figure}


The equilibrium results for the multi-peak scenario are more complex. In the numerical experiments, we consider a simplified case where the two groups and assume $t^*_{\tau_1} > t^*_{\tau_2}$. Then, the starting and ending time of rush hours are derived as 
\begin{align}
    \tstart &= \frac{1}{2}\left(t^*_{\tau_1} + t^*_{\tau_2} - \frac{N_{\tau_2}}{s}\right) - \frac{\gamma}{\beta+\gamma} \frac{N}{2s},\\
    \tend &= \frac{1}{2}\left(t^*_{\tau_1} + t^*_{\tau_2} + \frac{N_{\tau_1}}{s}\right) + \frac{\beta}{\beta+\gamma} \frac{N}{2s}.
\end{align}
The normalized equilibrium cost for each group reads, respectively,
\begin{align}
    c^*_{\tau_1} &= \frac{c^*}{2} + \frac{\gamma}{2}\left(t^*_{\tau_2} - t^*_{\tau_1} + \frac{N_{\tau_1}}{s}\right),\\
    c^*_{\tau_2} &= \frac{c^*}{2} +  \frac{\beta}{2}\left(t^*_{\tau_2} - t^*_{\tau_1} + \frac{N_{\tau_2}}{s}\right),
\end{align}
which implies that, by spreading out the desired arrival time, commuters can reduce their cost. 


\begin{remark}As a sanity check, consider the case that the two groups have independent departure windows but the ending time of first one equals the starting time of the other. Then, the equilibrium cost is $c^*_\tau = \frac{\beta\gamma}{\beta+\gamma} \frac{N_\tau}{s}$, and the desired arrival times satisfy
\begin{align}
    t^*_{\tau_1}-t^*_{\tau_2} = \frac{c^*_{\tau_1}}{\beta} + \frac{c^*_{\tau_2}}{\gamma}.
\end{align}
Above equations yield
\begin{align}
    c^*_{\tau_1} &= \frac{c^*}{2} + \frac{\gamma}{2}\left(-\frac{c^*_{\tau_1}}{\beta} - \frac{c^*_{\tau_2}}{\gamma} + \frac{\beta+\gamma}{\beta\gamma}c^*_{\tau_1}\right) = \frac{c^*}{2} - \frac{c^*_{\tau_2}}{2} + \frac{c^*_{\tau_1}}{2} = c^*_{\tau_1},\\
    c^*_{\tau_2} &= \frac{c^*}{2} + \frac{\beta}{2}\left(-\frac{c^*_{\tau_1}}{\beta} - \frac{c^*_{\tau_2}}{\gamma} + \frac{\beta+\gamma}{\beta\gamma}c^*_{\tau_2}\right) = \frac{c^*}{2} - \frac{c^*_{\tau_1}}{2} + \frac{c^*_{\tau_2}}{2} = c^*_{\tau_2}
\end{align}
\end{remark}
}


% Given the departure rate $\lambda_\textup{slow}(t)$, the queue is computed as $q(t)=\int_{t_\textup{start}}^t (\lambda_\textup{slow}(x) - \sslow)\mathrm{d}x$, where $t_\textup{start}$ is the time when the queue emerges (given below).
% % is the last time instant during which there was no queue, i.e., $q(\hat t) = 0$.}%and $p(t)$ is the toll price at time $t$. 

% Since the \gls{VOT} ratios are the same among all commuters, the departure rate on the slow lane follows the same pattern as in the homogeneous case.
% % In other words, travelers on the slow lane would randomly choose their departure time. %~\cite{xiao2013managing}. 
% According to \cite{sun:2020:managing_bn_incentives}[Eq.~7-10], 
% the starting and ending times of the peak hours ($\tstart$ and $\tend$), as well as the time with maximum queuing delay ($\tpeak$), read respectively
% \begin{align}
%     \label{eq:tstart-tend-tpeak}
%     \tstart_\rev \tau = t^*_\rev \tau-c^*_\rev \tau/\beta,\quad \tend_\rev \tau = t^*_\rev \tau+c^*_\rev \tau/\gamma,\quad \tpeak_\rev \tau = t^*_\rev \tau - c^*_\rev \tau/\alpha,
% \end{align}
% where
% \begin{align}
% \label{eq:classical-equilibrium-cost}
% c^*_\rev \tau = \frac{\beta\gamma}{\beta+\gamma} \: \frac{N}{s}
% \end{align}
% \rev{is the normalized slow lane equilibrium cost. TODO: verify how these equations are affected by heterogeneous $t^*$.}
% The equilibrium cost of each group on the slow lane is given by $c^*_j = u_j \: c^*$.


% \begin{figure}[htb]
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figures/model-eq.pdf}
% \caption{Equilibrium departures/arrivals on slow lane.}
% % \blue{at the equilibrium}.}
% \label{fig:model_eq}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figures/model-toll-disc.pdf}
% \caption{Optimal toll price $p^*(t)$ on fast lane.}
% \label{fig:model_toll}
% \end{subfigure}
% \caption{Illustration of equilibrium in base scenario with optimal pricing of the fast lane.}
% \label{fig:model}
% \end{figure}

% Figure~\ref{fig:model} illustrates the cumulative departures and arrivals on the slow lane, as well as the optimal toll price on the fast lane at equilibrium. The departure and arrival curves on the fast lane are omitted as they coincide with each other with constant rate $\sfast$.
% We follow a reasoning similar to~\cite{arnott1988schedule} to compute the optimal toll price $p^*(t)$ on the fast lane that leads to the social optimum. Consequently, the tolling policy is piece-wise linear and commuters with higher \gls{VOT} multipliers would depart closer to $t^*$ (see Figure~\ref{fig:model_toll}). 
% Letting $[t_j,t_{j+1}]$ and $[t'_{j+1}, t'_j]$ be the time intervals during which group $j$ enter the fast lane, the slope of the optimal toll price $p^*(t)$ satisfies
% \begin{align}\label{eq:toll_slope}
%     \dot p^*(t) = \begin{cases}
%         u_j \: \beta, & t\in[t_j,t_{j+1}], \\
%          -u_j \: \gamma, & t\in [t'_{j+1}, t'_j].
%     \end{cases}
% \end{align}
% % then the toll price satisfies
% % \begin{align}
% %     b(t) = \left\{\begin{array}{cc}
% %          u_j \beta (t-t_0), & t\in[t_j,t_{j+1}]\\
% %          -u_j \gamma (t-t_0) , & t\in [t'_{j+1}, t'_j]
% %     \end{array}\right..
% % \end{align}


% (the following may be moved to numerical experiments)
% With the starting/ending toll price equal to zero and the number of commuters in each group, the toll price at the boundary of each interval is given by
% \begin{align}
%     p(t_{j+1}) = p(t'_{j+1}) = \frac{\beta\gamma}{\beta+\gamma}\sum_{l=m}^j \frac{u_ln_l}{s_\textup{fast}},
% \end{align}
% where $n_l$ denotes the number travelers of group $l$ on the fast lane. % \footnote{The group size $n_l=p_lN$ except for group $m$.}



    
\subsection{Karma mechanism: theoretical framework}
\label{sec:karma-preliminaries}
In this section, we revisit the \emph{karma mechanism} firstly introduced in~\cite{elokda2022self}. In brief, it repeatedly allocates a resource to a group of competing agents over an infinite time horizon. 
\tbc{At each time step, an agent endowed with an integer quantity $k \in \Nat$, called \emph{karma}, can submit an integer bid $b \in \B[k]=\{0,\dots,k\}$ that cannot exceed the karma, hereafter referred to as a \emph{karma bid}.}
The resource is then allocated through an auction-like mechanism, and karma is transferred from the agents who acquire the resource to those who yield it in accordance to a \emph{karma payment and redistribution rule} to be designed.
% We recall the setting of \emph{karma mechanisms} as introduced in~\cite{elokda2022self}. In a karma mechanism, a common resource is repeatedly contested between competing agents over an infinite time. Each agent is endowed with an integer \emph{karma counter} $k \in \Nat$, and the resource is allocated in every time step using an auction-like mechanism where the competing agents each submit an integer \emph{karma bid} $b \in \B^k=\{0,\dots,k\}$ (the bid cannot exceed the karma of the agent). Subsequently, karma is transferred from the agents that acquire the resource to those who yield it, in accordance to a \emph{karma payment and redistribution rule} that is free to design.
Apart from the karma, each agent also features an \emph{urgency state} $u \in \U=\{u_1,\dots,u_M\}$, $u>0$.
It describes the urgency to acquire the resource (e.g., the \gls{VOT} in a morning commute scenario).
Given a finite number of agent types $\tau \in \Gamma\subset \Nat$, the urgency of an agent of type $\tau$ evolves according to an exogenous
% and \gls{iid}
Markov chain, denoted by $\phi_\tau[u^+ \mid u]$.
% Moreover, each agent has a (possibly) time-varying need for the resource which we represent by the \emph{urgency state} $u \in \U = \{u_1,\dots,u_{n_u}\}$.
% The urgency state typically multiplies the immediate cost for failing to acquire the resource (e.g., to model the sensitivity of the agent towards delays as a function of the trip purpose).
% It evolves in time according to an exogenous Markov chain that is independent for each agent, denoted by $\phi[u^+ \mid u]$.
The principle of a karma mechanism is to facilitate a fair and efficient allocation of the resource. Specifically, it incentivizes agents to save karma for periods of high urgency and thus enables the resource to be assigned to those who need it the most. 
% The main working principle of a karma mechanism is that it both facilitates a form of fair turn taking through the karma transfers, as well as incentivizes agents to spare karma for periods of high urgency, which contributes to highly efficient resource allocations (i.e., allocations where the resource is acquired by those who need it most).

Formally, the karma mechanism is modeled as a \emph{dynamic population game}~\cite{elokda2021dynamic}. Namely, the number of agents $N$ is assumed large, thus they can be approximated by a continuum of mass.
The distribution of agent types is compactly denoted by $g\in\Delta(\Gamma)$, where $g_\tau\in[0,1]$ is the mass of agents in type $\tau\in\Gamma$.
% Formally, we consider that the number of agents $N$ is large such that they approximately form a continuum of mass, and model karma mechanisms as \emph{dynamic population games}~\cite{elokda2021dynamic}.
% In the karma dynamic population game, agents are grouped by \emph{static types} $\tau \in \Gamma = \{\tau_1,\dots,\tau_{n_\tau}\}$ and \emph{dynamic states} $x = (u,k) \in \X = \U \times \Nat$.
% The state consists of the urgency state $u$ and the karma $k$ of the agent.
% The distribution of agents in each type is given by the static parameter $g \in \Delta(\Gamma)$, with $g_\tau$ denoting the mass of agents in type $\tau$.
Accordingly, the time-varying joint \emph{type-state distribution} is given by
\begin{align}
    d \in \D = \left\{d \in \Real_+^{|\Gamma| \times |\X|} \left\lvert \; \sum_{u,k} d_\tau[u,k] = g_\tau, \quad \forall \tau \in\Gamma \right. \right\},
\end{align}
where $d_\tau[u,k]$ denotes the mass of agents in the \emph{static type} $\tau$ and \emph{dynamic state} $[u,k] \in \X$, and $\X = \U \times \Nat$.

At each time step, each agent can choose an action $a$ from a finite state-dependent discrete set $\A[u,k]$. The action includes the agent's bid $b$ as well as other decisions, e.g., the departure time in a morning commute scenario.
% At each time step, agents can play an action $a \in \A^x$, where $\A^x$ is a (possibly) state-dependent discrete action set.
% Typically in a karma mechanism, the action is the bid $b$ of the agent, but one consider other kinds of actions as well (such as the departure time during the rush hour).
Agents of the same type $\tau$ follow the homogeneous randomized policy 
$\pi_\tau : \X \rightarrow \Delta(\A[u,k])$,
% $\pi_\tau : \X \rightarrow \Delta(\A^x)$\todo{\footnote{\todo{Slight abuse of notation here}}
% }, 
where $\pi_\tau[a \mid u,k]$ denotes the probabilistic weight that these agents place on action $a$ when in state $[u,k]$.
The concatenation of the policies of all types 
$\pi = (\pi_\tau)_{\tau\in\Gamma}$
% $\pi = (\pi_{\tau_1},\cdots,\pi_{\tau_{n_\tau}})$ 
is simply referred to as the \emph{policy}, and the space of policies is denoted by $\Pi$. 


\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{figures/karma-transit.pdf}
\caption{One-step state transition of an agent of type $\tau$. \rev{TODO: $\kappa$ does not depend on $u$.}}
\label{fig:karma_transit}
\end{figure}



In the dynamic population game, the tuple of type-state distribution and policy $(d,\pi)$ is referred to as the \emph{social state} because it gives a macroscopic description of the distribution of agents in the population as well as their behaviors. Hence, all the outcomes at each time step are functions of $(d,\pi)$. 
Let $\kappa[k^+ \mid k,a](d,\pi)$ be the \emph{karma transition function} that describes how the agent's karma changes between two consecutive time steps given its current karma $k$ and action $a$. Then, together with the urgency transition function $\phi_\tau[u^+ \mid u]$, the joint \emph{state transition function} is given by
% The pair of type-state distribution and policy $(d,\pi)$ is an important quantity which we refer to as the \emph{social state}.
% The social state $(d,\pi)$ gives a macroscopic description of the distribution of agents in the population as well as how the agents behave.
% At each time step, each agent experiences an \emph{immediate reward} given by
% \begin{align}
%     \label{eq:immediate-reward}
%     \zeta[u,a](d,\pi).
% \end{align}
% In general, the immediate reward depends on the urgency state $u$ of the agent, the agent's own action $a$, as well as the behavior of other population agents encoded in the social state $(d,\pi)$.
% Moreover, the agent's karma transitions according to a \emph{karma transition function}
% \begin{align}
%     \label{eq:karma-transition}
%     \kappa[k^+ \mid k,a](d,\pi),
% \end{align}
% which, together with the exogenous urgency transitions $\phi[u^+ \mid u]$, yields the following joint \emph{state transition function}
\begin{align}
    \label{eq:state-transition}
    \rho_\tau[u^+, k^+ \mid u,k,a](d,\pi) = \phi_\tau[u^+ \mid u] \: \kappa[k^+ \mid k, a](d,\pi).
\end{align}
% In words, $\kappa[k^+ \mid k,a](d,\pi)$ gives the probability of transitioning from karma $k$ to $k^+$ when playing action $a$ in the current time step.
% In general, these transition probabilities are a function of the behavior of other population agents (encoded in $(d,\pi)$) as well as the karma payment and redistribution rules in place.
Figure~\ref{fig:karma_transit} illustrates a one-step state transition of an agent of type $\tau$.
% \blue{and introduces the karma and urgency transition functions $\kappa$ and $\phi$, respectively}. 
Moreover, we define $\zeta_\rev{\tau}[u,a](d,\pi)$ as the \emph{immediate reward function} of each \rev{type $\tau$} agent in urgency $u$ taking action $a$. Both the immediate reward and the karma transition will be further specified in Section~\ref{sec:karma-bottleneck}. Yet, two conditions are required to ensure that the karma mechanism is well defined.
% In Section~\ref{sec:karma-bottleneck}, our main task will be to derive the specifics of the immediate reward function~\ref{eq:immediate-reward} and the karma transition function~\ref{eq:karma-transition} in the proposed karma-based bottleneck management scheme, and to verify that they satisfy the following two high-level properties which are needed for the well-posedness of the problem.

% \begin{assumption}[Continuity]
% \label{as:continuity}
% The immediate reward function~\ref{eq:immediate-reward} and the karma transition function~\ref{eq:karma-transition} are continuous in the social state $(d,\pi)$.
% \end{assumption}

\begin{assumption}[Continuity]
\label{as:continuity}
The immediate reward function $\zeta_\rev{\tau}[u,a](d,\pi)$ and the 
karma transition function $\kappa[k^+ \mid k,a](d,\pi)$ are continuous in the social state $(d,\pi)$.
\end{assumption}

\begin{assumption}[Karma preservation in expectation]
\label{as:karma-preservation}
Karma is preserved in expectation for all $(d,\pi)$, i.e., $\E[k^+] = \E[k]$,
% \begin{align}
%     \E_{\substack{(\tau,u,k) \sim d, \;a \sim \pi_\tau[\cdot \mid u,k]}}[k^+] = \E_{(\tau,u,k) \sim d}[k],
% \end{align}
which expands to
\begin{align}    
    \sum_{\tau,u,k} d_\tau[u,k] \sum_a \pi_\tau[a \mid u,k] \sum_{k^+} \kappa[k^+ \mid k,a](d,\pi) \: k^+ = \sum_{\tau,u,k} d_\tau[u,k] \: k.  \label{eq:karma-preservation}
\end{align}
\end{assumption}
In brief, Assumption~\ref{as:karma-preservation} requires that the total amount of karma in the system remains the same, i.e., the amount paid by agents equals the amount received by agents. The readers are referred to~\cite{elokda2022self} for an in depth discussion on the assumptions and functions introduced above.
% Intuitively, Assumption~\ref{as:karma-preservation} requires that the karma held by the population agents is preserved (i.e., the total amount of karma paid equals the total amount of karma received in the population).
% Refer to~\cite{elokda2022self} for an in depth discussion of Assumption~\ref{as:continuity}--\ref{as:karma-preservation}.

Given the social state, each agent  faces a \emph{Markov decision process}. 
Specifically, the expected reward of the agents of type $\tau$ is given by 
\begin{align}
    R_\tau[u,k](d,\pi) = \sum_a \pi_\tau[a \mid u,k] \: \zeta_\rev{\tau}[u,a](d,\pi),
\end{align}
and the state transition follows 
\begin{align}
    P_\tau[u^+,k^+ \mid u,k](d,\pi) = \sum_a \pi_\tau[a \mid u,k] \: \rho_\tau[u^+,k^+ \mid u,k,a](d,\pi).
\end{align}
Accordingly, the expected return in the infinite horizon, also known as the value function, is derived as 
\begin{align}\label{eq:value-function}
    V_\tau[u,k](d,\pi) = R_\tau[u,k](d,\pi) + \delta \sum_{u^+,k^+} P_\tau[u^+,k^+ \mid u,k](d,\pi) \: V_\tau[u^+,k^+](d,\pi),
\end{align}
where $\delta\in(0,1]$ is the discount factor. A smaller $\delta$ models a more myopic agent behavior.
To describe the rational decision of each agent, we also need to define the state-action value function, also called $Q$-function, as
\begin{multline}
    \label{eq:Q-function}
    Q_\tau[u,k,a](d,\pi) \\
    = \zeta_\rev{\tau}[u,a](d,\pi) + \delta \sum_{u^+,k^+} \rho_\tau[u^+,k^+ \mid u,k,a](d,\pi) \: V_\tau[u^+,k^+](d,\pi).
\end{multline}
Then, to maximize the long-term return, each agent chooses a policy based on the \emph{best response} correspondence, given by 
\begin{multline}
    B_\tau[u,k](d,\pi) = \left\{\sigma \in \Delta(\A(u,k)) \left \lvert \; \forall \sigma' \in \Delta(\A(u,k)), \vphantom{\sum_a} \right. \right.\\
    \left. \sum_a (\sigma[a] - \sigma'[a]) \: Q_\tau[u,k,a](d,\pi) \geq 0 \right\}.
\end{multline}
By definition, $B_\tau[u,k](d,\pi)$ gives the set of randomized individual actions that maximize the $Q$-function in state $[u,k]$ for agents of type $\tau$.

% The immediate reward function~\ref{eq:immediate-reward} and the state transition function~\ref{eq:state-transition} jointly define a \emph{Markov decision process} (MDP) that each agent faces, and the MDPs of different agents are coupled through the social state $(d,\pi)$.
% We now turn to characterize a suitable notion of equilibrium in this setting, for which we need the following derivations.
% We consider that the agents discount their future rewards with the discount factor $\delta \in [0,1)$.
% An agent following the policy of its type $\pi_\tau$ experiences an expected immediate reward of
% \[
%     R_\tau[u,k](d,\pi) = \sum_a \pi_\tau[a \mid u,k] \: \zeta[u,a](d,\pi),
% \]
% and the state of the agent transitions according to the stochastic matrix
% \[
%     P_\tau[u^+,k^+ \mid u,k](d,\pi) = \sum_a \pi_\tau[a \mid u,k] \: \rho[u^+,k^+ \mid u,k,a](d,\pi).
% \]
% The agent's expected infinite horizon reward (commonly known as the value function) is therefore recursively defined as
% \[
%     V_\tau[u,k](d,\pi) = R_\tau[u,k](d,\pi) + \delta \sum_{u^+,k^+} P_\tau[u^+,k^+ \mid u,k](d,\pi) \: V_\tau[u^+,k^+](d,\pi),
% \]
% which is the well-known Bellman recursion for the fixed policy $\pi_\tau$.
% The agent's \emph{single-stage deviation reward} (commonly known as the Q-function) is given by
% \[
%     Q_\tau[u,k,a](d,\pi) = \zeta[u,a](d,\pi) + \alpha \sum_{u^+,k^+} \rho[u^+,k^+ \mid u,k,a](d,\pi) \: V[u^+,k^+](d,\pi).
% \]
% This is the expected infinite horizon reward when the agent deviates from $\pi_\tau$ for a single time step by playing $a$ in state (u,k), then follows $\pi_\tau$ in the future.
% The \emph{state-dependent best response} correspondence is hence given by
% \[
%     B_\tau[x](d,\pi) \in \left\{\sigma \in \Delta(\A^x) \left \lvert \; \forall \sigma' \in \Delta(\A^x), \; \sum_{a} (\sigma[a] - \sigma'[a]) \: Q_\tau[x,a](d,\pi) \geq 0 \right. \right\}.
% \]
% This is the set of randomized actions maximizing the expected single-stage deviation reward of an agent in state $x=(u,k)$.
% We are finally ready to state the definition of the equilibrium in our setting.


We are finally ready to define the equilibrium state under a karma mechanism.
\begin{definition}[\gls{SNE}]
\label{def:SNE}
A \acrlong{SNE} is a social state $(d^*,\pi^*) \in \D \times \Pi$ such that, for all $[\tau,u,k] \in \Gamma \times \U \times \Nat$,
\begin{align}
    d^*_\tau[u,k] &= \sum_{u^-,k^-} d^*_\tau[u^-,k^-] \: P_\tau[u,k \mid u^-,k^-](d^*,\pi^*), \label{eq:SNE-1} \\
    \pi^*_\tau[\cdot \mid u,k] &\in B_\tau[u,k](d^*,\pi^*). \label{eq:SNE-2} 
\end{align}
% \begin{align}
%     \sd_\tau[u,k] &= \sum_{u^-,k^-} \sd_\tau[u^-,k^-] \: P_\tau[u,k \mid u^-,k^-](\sd,\epi), \label{eq:SNE-1} \tag{SNE.1} \\
%     \epi_\tau[\cdot \mid u,k] &\in B_\tau[u,k](\sd,\epi). \label{eq:SNE-2} \tag{SNE.2}
% \end{align}
\end{definition}
\tbc{The \gls{SNE} is similar to the classical notion of Nash equilibrium in that it denotes a state of the game where all agents have no incentive to unilaterally deviate from the equilibrium policy $\pi^*$ given by Eq.~\ref{eq:SNE-2}, but it  additionally requires that the type-state distribution $d^*$ is \emph{stationary} 
% under the stochastic processes characterized by the stochastic matrix $P_\tau[u^+,k^+ \mid u,k](\sd,\epi)$
as per Eq.~\ref{eq:SNE-1}.}

We conclude this section by stating the conditions for a karma mechanism to guarantee the existence of a \gls{SNE}  
% We conclude this section by stating the main result on the well-posedness of karma mechanisms which guarantees that a stationary Nash equilibrium exists 
(see~\cite{elokda2022self} for the proof).
\begin{theorem}[Existence of \acrlong{SNE}, \cite{elokda2022self}~Theorem~1]
\label{th:Nash-exists}
If Assumptions~\ref{as:continuity} and~\ref{as:karma-preservation} hold, then, given $\bar{k} \in \Nat$, there always exists a \gls{SNE} $(d^*,\pi^*)$ such that $\sum_{\tau,u,k} d^*_\tau[u,k] \: k = \kbar$, and $\kbar$ is the average amount of karma per agent in the system.
% Let Assumption~\ref{as:continuity} and~\ref{as:karma-preservation} hold. Then for each $\bar{k} \in \Nat$, a stationary Nash equilibrium $(\sd,\epi)$ satisfying $\sum_{\tau,u,k} \sd_\tau[u,k] \: k = \kbar$ is guaranteed to exist.
\end{theorem}
% Note that $\kbar$ is the average amount of karma in the system, a parameter that is free to design.

